Is Pure Exploitation Sufficient in Exogenous MDPs with Linear Function Approximation?

Exogenous MDPs (Exo-MDPs) capture sequential decision-making where uncertainty comes solely from exogenous inputs that evolve independently of the learner's actions. This structure is especially common in operations research applications such as inventory control, energy storage, and resource allocation, where exogenous randomness (e.g., demand, arrivals, or prices) drives system behavior. Despite decades of empirical evidence that greedy, exploitation-only methods work remarkably well in these settings, theory has lagged behind: all existing regret guarantees for Exo-MDPs rely on explicit exploration or tabular assumptions. We show that exploration is unnecessary. We propose Pure Exploitation Learning (PEL) and prove the first general finite-sample regret bounds for exploitation-only algorithms in Exo-MDPs. In the tabular case, PEL achieves $\widetilde{O}(H^2|\Xi|\sqrt{K})$. For large, continuous endogenous state spaces, we introduce LSVI-PE, a simple linear-approximation method whose regret is polynomial in the feature dimension, exogenous state space, and horizon, independent of the endogenous state and action spaces. Our analysis introduces two new tools: counterfactual trajectories and Bellman-closed feature transport, which together allow greedy policies to have accurate value estimates without optimism. Experiments on synthetic and resource-management tasks show that PEL consistently outperforming baselines. Overall, our results overturn the conventional wisdom that exploration is required, demonstrating that in Exo-MDPs, pure exploitation is enough.

==> iclr2026/backup_text.tex <==



\section{Numerical experiments}
\label{sec:exp}

\subsection{Tabular Exo-MDP}
\label{sec:exp-tab}

\noindent
\begin{minipage}[t]{0.60\textwidth}
\paragraph{Setup.}  We evaluate on synthetic tabular Exo-MDPs with endogenous state space \(\mathcal{X}=[5]\), exogenous state space \(\Xi=[5]\), and action set \(\mathcal{A}=[3]\) and horizon \(T=5\), and \(K=250\) episodes. Rewards are drawn i.i.d.\ as \(r(x,a,\xi)\sim\text{Unif}(0,1)\). Endogenous dynamics are deterministic, 
\(
x_{h+1}=f(x_h,a_h,\xi_{h+1})=(x_h+a_h+\xi_{h+1})\bmod X,
\) 
while the exogenous process is a Markov chain with transition matrix \(P_y\) sampled row-wise from a Dirichlet prior.

% We evaluate on synthetic tabular Exo-MDPs with endogenous state space \(\mathcal X=[X]\), exogenous space \(\Xi=[Y]\) and action set \(\mathcal A=[A]\) with the default parameters
% \(X=5\), \(Y=5\), \(A=3\), horizon \(T=5\), and \(K=100\) episodes. %(averaged over \(L\) runs, \(L=1\) unless stated)
% Rewards are drawn i.i.d.\ \(r(x,a,\xi)\sim\text{Unif}(0,1)\). Endogenous dynamics are deterministic $x_{h+1}=f(x_h,a_h,\xi_{h+1})=(x_h+a_h+\xi_{h+1})\bmod X$,
% while the exogenous process is a Markov chain with transition matrix \(P_y\) sampled row-wise from a Dirichlet prior.  \srscomment{What is the $X$ in the $\bmod X$?}

\paragraph{Comparisons.} We compare \pto with its optimistic counterpart \texttt{PTO-Opt}, which replaces the empirical model $\hat{\bP}^k$ by an optimistic model $\tilde{\bP}^k$ in the Bellman backup. 
\end{minipage}\hfill
\begin{minipage}[t]{0.36\textwidth}
\centering
\vspace*{-\baselineskip}
\includegraphics[width=\linewidth]{iclr2026/figs/regret_comparison_c0.3.png}
\captionof{figure}{Comparison between \pto and \texttt{PTO-Opt}.}
\label{fig:tab}
\end{minipage}

Figure~\ref{fig:tab} illustrates the benefit of exploiting the observed exogenous trace. Despite no explicit exploration, \pto outperforms the exploration-heavy baseline \texttt{PTO-Opt} in cumulative regret.


\subsection{Storage control}
\label{sec:exp-adp}


\paragraph{Setup.} We consider a storage control setting where $x_h \in \cX=[0, C]$ denotes the current storage level. After taking action $a_h \in \mathcal{A}=[-a_{\max},a_{\max}]$, the system transitions to the post-decision state $x_h^{a} = f^{a}(x_h,a) = \mathrm{clip}_{[0,C]}\!\left(x_h + \eta^{+}a^{+} - \tfrac{1}{\eta^{-}}a^{-}\right)$. The exogenous component is the discrete price. The storage level is modeled as $x_{h+1}=g(x_h^{a},\xi_{h+1})=\alpha\,x_h^{a}, \alpha\in(0,1]$,
with default $\alpha=1$. The reward function is $r(x_h,a_h,\xi_h) = -\xi_h a_h - \alpha_c |a_h| - \beta_h x_h$,
capturing the market transaction, transaction cost, and holding penalty respectively. 


% We consider a storage setting where $x_h \in \cX=[0, C]$ is the storage level. After taking an action $a_h \in \mathcal{A}=[-a_{\max},a_{\max}]$, 
% the system transitions to a post-decision state $x_h^{a} = f^{a}(x_h,a) 
% = \mathrm{clip}_{[0,C]}\!\left(x_h + \eta^{+}a^{+} - \tfrac{1}{\eta^{-}}a^{-}\right)$, which enforces the capacity constraint. The exogenous component is the discrete price.% drawn from a discrete set $\Xi=\{\zeta_1,\dots,\zeta_R\}$. 
% %From the observed price trajectories $\{\xi_h^{\,\ell}\}$, we construct an 
% %empirical Markov model $\hat P(\xi'|\xi)$ to approximate the price dynamics. 
%  The storage level may be subject to leakage, modeled as $x_{h+1}=g(x_h^{a},\xi_{h+1})=\alpha\,x_h^{a}, \alpha\in(0,1]$ with default $\alpha=1$. The reward function is defined as $r(x_h,a_h,\xi_h) = -\xi_h a_h - \alpha_c |a_h| - \beta_h x_h$, capturing the market transaction, transaction cost, and holding penalty respectively. 

\paragraph{Features and anchors.} We discretize $\cX$ using anchors $\rho_n=\tfrac{n-1}{N-1}C$ for $n\in[N]$. A one-dimensional hat basis is employed: for any $x^a$, the feature vector $\phi(x^a)\in\mathbb{R}^N$ has at most two nonzero entries. Let $\Delta=\rho_{j+1}-\rho_j$. If $x^a \in [\rho_j,\rho_{j+1}]$, then $\phi_{j}(x^{a}) = \frac{\rho_{j+1}-x^{a}}{\Delta}, \phi_{j+1}(x^{a}) = \frac{x^{a}-\rho_j}{\Delta}$,
with all other coordinates zero. At anchor points, the basis reduces to canonical vectors, $\phi(\rho_n)=e_n$, so that $\Phi_h = I_N$ and $\Sigma_h=\Phi_h\Phi_h^\top=I_N$.

% We discretize $\cX$ using anchors $\rho_n=\tfrac{n-1}{N-1}C$ for $n\in[N]$. A one-dimensional hat basis is employed: for any $x^a$, the feature vector $\phi(x^a)\in\mathbb{R}^N$ has at most two nonzero entries. Let $\Delta=\rho_{j+1}-\rho_j$. If $x^a \in [\rho_j,\rho_{j+1}]$, then
%  Let $\Delta=\rho_{j+1}-\rho_j$.
% If $x^a \in [\rho_j,\rho_{j+1}]$, then $\phi_{j}(x^{a}) = \frac{\rho_{j+1}-x^{a}}{\Delta}$ and $\phi_{j+1}(x^{a}) = \frac{x^{a}-\rho_j}{\Delta}$ 
% with all other coordinates equal to zero. At anchor points, the basis 
% reduces to the canonical vectors, $\phi(\rho_n)=e_n$, so that  $\Phi_h = I_N$, and $\Sigma_h=\Phi_h\Phi_h^\top=I_N$.

\paragraph{Comparisons.} In \Cref{fig:cosine_analysis} we compare \lsvi with optimism-based exploration \texttt{LSVI-Opt}. Across all instances, \lsvi consistently outperforms \texttt{LSVI-Opt}, emphasizing that in Exo-MDPs exploitation strategies dominate optimism-based ones.

\begin{figure}[h]
    \centering
    % left
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{iclr2026/figs/cumulative_gap_ep100_T6_R10_K10_c0.5.png}
        \caption{$H=6$}
        \label{fig:cosine_hist}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{iclr2026/figs/cumulative_gap_ep100_T8_R10_K10_c0.5.png}
        \caption{$H=8$ }
        \label{fig:cosine_hist}
    \end{subfigure}
    \hfill
    % right
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{iclr2026/figs/cumulative_gap_ep100_T10_R10_K10_c0.5.png}
        \caption{$H=10$}
        \label{fig:cosine_cdf}
    \end{subfigure}
    \caption{Comparison of \lsvi and \texttt{LSVI-Opt} across three different time horizon lengths. 
    }
    \label{fig:cosine_analysis}
    \vspace{-4ex}
\end{figure}



\begin{comment}
% --- Storage Setup ---
\begin{itemize}[leftmargin=*]  
  \item \textbf{Endogenous pre-decision state:} $x_h \in [0, C]$.
  \item \textbf{Endogenous post-decision state:}
  \[
  x_h^{a} \;=\; f^{a}(x_h,a)
  \;=\; \mathrm{clip}_{[0,C]}\!\left(x_h+\eta^{+}a^{+}-\frac{1}{\eta^{-}}a^{-} \right).
  \]
  \item \textbf{Exogenous price:} discrete price set
  $\Xi=\{\zeta_1,\dots,\zeta_R\}$; estimate a Markov matrix
  $\hat P(\xi' \mid \xi)$ from the dataset $\{\xi_h^{\,\ell}\}$ 
  \item \textbf{Leakage (optional):}
  \[
  x_{h+1}=g(x_h^{a},\xi_{h+1})=\alpha\,x_h^{a}
  \quad\text{with } \alpha\in(0,1].
  \]
  \item \textbf{Reward:}
  \[
  r(x_h,a_h,\xi_h) \;=\; -\xi\,a_h \;-\; \alpha_c |a_h| \;-\; \beta_h x_h.
  \]
  \item \textbf{Actions:} interval
  $\mathcal{A}=[-a_{\max},a_{\max}]$ 
  \item \textbf{Anchors (post-decision grid):}
  \[
  \rho_n=\frac{n-1}{N-1}\,C,\qquad n\in[N].
  \]
  \item \textbf{Feature map (1D hat basis):} for any $x^{a}$, $\phi(x^{a})\in\mathbb{R}^{N}$ has at most two nonzeros.
  \begin{itemize}
    \item If $x^{a}\in[\rho_j,\rho_{j+1}]$, then
    \[
    \Delta=\rho_{j+1}-\rho_{j}, \quad \phi_{j}(x^{a})=\frac{\rho_{j+1}-x^{a}}{\Delta},\qquad
    \phi_{j+1}(x^{a})=\frac{x^{a}-\rho_{j}}{\Delta},    
    \]
    and others are $0$.
  \end{itemize}
  At anchors, $\phi(\rho_n)=e_n\;\Rightarrow\; \Phi_h=I_N\;\Rightarrow\; \Sigma_h=\Phi_h\Phi_h^\top=I_N$.
\end{itemize}
\end{comment}

% \section{Conclusions} \label{sec:con}
% \hao{TODO}
% \srscomment{Don't stress about this, you can get rid of it if you want}









\begin{comment}

\section{Tabular Exo-MDPs}
\label{sec:wm}

\subsection{Warm-up: exogenous multi-armed bandits}
\label{sec:mab}

\srscomment{Couple comments on this section as written that we can discuss when we meet tomorrow. First, \pel isn't defined yet, so the first introduction to it is a bit forward looking. Second, I don't think you need a {\em formal} definition of the MAB set-up. All you need to do is specify this as an Exo-MDP with $H = 1$ and no states, and then you have all of the notation that you need directly right?  I think you can call this an ``Exo-Bandit'', I think we refer to this set-up like that in \citet{wan2024exploiting}.}

\srscomment{Oh, realizing in hindsight you are using \pel as any ``pure exploitation algorithm'', instead of to refer to a specific algorithm}


\srscomment{Can cut from here}
As a warmup, we consider stochastic MABs with exogenous information and prove that \pel attains optimal regret bound. We start with revisiting the stochastic MAB.
\paragraph{Stochastic MAB.} There are arms $a\in[A]$, $A\ge 2$. At each round $k=1,2,\dots,K$, the agent selects $a_k$ and observes a stochastic reward $R_h\in[0,1]$ with $\mathbb{E}[R_k\,|\,a_k=a]=\mu_a$. Let $\mu^\star=\max_{a}\mu_a$ and define the simple regret for round $k$ and the cumulative regret over $K$ rounds
\begin{align*}
    \sr{k}\;=\;\mathbb{E}\!\left[\mu^\star-\mu_{a_k}\right], \quad \mathrm{Regret}(K)\;=\;\mathbb{E}\!\left[\sum_{k=1}^K\bigl(\mu^\star-\mu_{a_k}\bigr)\right].
\end{align*}
Now we consider MAB with exogenous information. In round $k$, the agent pulls the arm $a_k$ and observes $\xi_k$, and receives the reward $R_k=r(a_k,\xi_k)$, where $r:\cA\times\Xi\mapsto\bR$ is the \emph{known} reward function, and $\xi_k$ is the unknown i.i.d. exogenous variable.  Therefore, the agent can receive the rewards for all arms $r(a,\xi_k)_{a\in[A]}$ in each round, even if a particular $a_k$ is chosen before. This is exactly the MAB with full information, which is different from the partial feedback setting where the agent can only observe the reward for chosen $a_k$.  \srscomment{To here}
\srscomment{Right, MABs with full feedback have been studied before in the literature (just under ``experts'' or ``bandits with full feedback.''.  }

Under the Exo-MAB setting, \ftl specifies to the Follow-The-Leader (\ftl), which pulls in each round the arm with the highest empirical mean. Let $\hat{\mu}_{a}(k):=\frac{1}{k-1}\sum_{s=1}^{k-1}r(a,\xi_s)$, \ftl chooses $a_k=\arg\max_{a\in [A]}\hat{\mu}_{a}(k)$. Without loss of generality, we assume $\mu^{\star}=\mu_1>\mu_j, \forall 1<j\leq A$. 
\begin{proposition}%[Regret bound of \ftl for Exo-MAB]
\label{prop:ftl_mab}
    The expected simple regret and of \ftl for Exo-MAB  with $A$ arms satisfies
    \[ \sr{\ftl,k}  \leq \sqrt{2\sigma^2\log A/(k-1)},\]
    and thus the expected cumulative regret 
    \[ \rgr{\ftl,K}  \leq 2\sigma\sqrt{(K-1)\log A}. \]
\end{proposition}
\textbf{[TODO]: Add the regret lower bound in Exo-MAB.} 
\srscomment{Right, none of these results are really new though?}

\srscomment{What is \pel vs \ftl in this context?}
In contrast to \pel, optimism-based exploration are the well-known methods that attains optimal regret bounds for MAB, among which Upper Confidence Bound (\texttt{UCB}) is the most standard practice. We provide the regret upper bound of \ucb for Exo-MAB.
\begin{proposition}%[\texttt{UCB} with full information]
\label{prop:}
    The  expected cumulative regret of \texttt{UCB} in the Exo-MAB setting with $A$ arms satisfies
    \[ \rgr{\texttt{UCB},K}  \leq \sqrt{2\sigma^2\log(AK^2)(K-1)} + \mathcal{O}(1). \]
\end{proposition}
\ftl is minimax optimal, which improves \texttt{UCB} by an additive factor of $\mathcal{O}(\sigma\sqrt{K\log K})$. Therefore, Optimism is not helpful, but could be harmful, while \pel alone suffices. %\textbf{[TODO]: Add comparison figures \pel vs. \ucb/TS.} 
\srscomment{Yeah, I guess it's a bit tough to understand what exactly the point of this section is. Not entirely certain it adds too much. If the story is just that when you specialize the algorithm to an Exo-Bandit you recover existing results in the literature? Or are you trying to use it as a warm-up to define the algorithm? At the moment the writing is just kind of presenting some propositions without getting into why we should care about this specific section as a warm-up.}

\subsection{Tabular Exo-MDPs}
\label{sec:tab}
Now we consider the tabular Exo-MDP setting, where the the state and action size are finite. \ftl can be extended to tabular Exo-MDP setting. Observe that
$V^{\pi}_1(s_1) = \mathbb{E}_{\boldsymbol{\xi}}\left[V_1^\pi\left(s_1, \boldsymbol{\xi}\right)\right]$ and the distribution of $\bxi$ is independent of $\pi$. Using the exogenous trace $\bxi^k$ up to episode $k$, we obtain the universally unbiased estimator of the value function
\[ \widetilde{V}_1^{k,\pi}(s_1):=%\overline{\mathbb{E}}\left[V_1^\pi\left(x_1, \boldsymbol{\xi}\right)\right]:=
\frac{1}{k} \sum_{l=1}^k V_1^\pi\left(s_1, \boldsymbol{\xi}^l_{>1}\right) = \frac{1}{k} \sum_{l=1}^k \sum_{h=1}^H r(x_h,\pi_h(s_h),\xi^l_{h}), \]
which is unbiased for any policy $\pi$. %Note that $V_1^\pi(x_1, \cdot)$ can be evaluated for any policy and any $\xi$ by (deterministic) forward simulation
%\[ x_{h+1} = f(x_h,a_h,\xi_h), \ a_{h} = \pi_h(x_{h},\xi_h).  \]
\ftl chooses the greedy policy w.r.t. the empirical value function: $\tilde{\pi}^k:=\arg \max_{\pi \in \Pi} \widetilde{V}_1^{k,\pi}(s_1).$
By extending the proof from Exo-MAB, we obtain the regret bounds of \ftl for Exo-MDP. \srscomment{Should add comment that this is equivalent to the ``ERM'' algorithm from \citet{sinclair2023hindsight}}
\begin{proposition}[Theorem 7 in \cite{sinclair2023hindsight}]
Given any $\delta \in(0,1)$, with probability at least $1-\delta$, 
$$
\sr{\ftl,K} \leq H\sqrt{\frac{2  \log (2|\Pi| / \delta)}{K}} = H\sqrt{\frac{2  H|\mathcal{X}||\Xi|\log (A / \delta)}{K}}.
$$
Furthermore,
$$
\bE[\sr{\tilde{\pi},K}] \leq H\sqrt{\frac{ \log |\Pi|}{K}} = H\sqrt{\frac{  H|\mathcal{X}||\Xi|\log (A )}{K}}.
$$
\end{proposition}
\srscomment{Using new notation here, was $\rgr{\texttt{alg},K}$ before, now sr?}
The proof follows by extending from Exo-MAB setting. While \ftl attains near-optimal regret for Exo-MDP, it is computationally inefficient since there is no dynamic programming structure for \ftl in general. Specifically, to obtain the exact optimal policy in general, \ftl needs to perform an exhaustive search, which incurs computational complexity  $\cO(A^{SH} (K + HS\log A)$ (evaluation and sorting).
\begin{remark}
Markovian vs. i.i.d. exogenous processes, and general [].     
\end{remark}
To avoid the computational inefficiency, an alternative \pel approach Predict Then Optimize (\pto) learns the transition model $\widehat{\bP}_h$ as approximation of the true distribution $\bP_h$, and uses $\widehat{\bP}$ to efficiently solve the Bellman equation. In particular, \pto
uses  the empirical distribution $\widehat{\bP}^k_h\left(\xi_{h+1} \mid \xi_{h}\right):= \sum_{l=1}^{k-1} \bI \cbrk{\xi^l_{h}=\xi_{h},\xi^l_{h+1}=\xi_{h+1}}/\sum_{l=1}^{k-1} \bI \cbrk{\xi^l_{h}=\xi_{h}}$ to implement the Bellman backup
$$
\begin{aligned}
\widehat{Q}^k_h(s_h, a_h) & :=r(x_h, a_h, \xi_{h}) + \mathbb{E}_{\xi_{h+1} \mid \xi_{h}}\left[\widehat{V}_{h+1} \prt{f(x_h, a_h, \xi_{h+1}),\xi_{h+1}} \mid s_h,a_h;\widehat{\bP}^k_h\right] \\
%&=:\hat{\mathbb{E}}_{\xi_{h+1} \mid \xi_{h}}\left[r(x_h, a_h, \xi_h)+\widehat{V}_{h+1} \prt{f(x_h, a_h,\xi_h),\xi_{h}} \right] \\
 \widehat{\pi}^k_h(s_h)  &:=\underset{a_h \in \mathcal{A}}{\arg \max} \ \widehat{Q}^k_h(s_h, a_h), \widehat{V}^k_h(s_h)  := \widehat{Q}^k_h(s_h, \widehat{\pi}^k_h(s_h)).
\end{aligned}
$$
%One limitation is that for \textit{non-Markovian} DP, the empirical distribution may become very sparse as $h$ increases, leading to large variance.
\begin{proposition}[Adapted Theorem 6 in \cite{sinclair2023hindsight}]
Suppose that for some $k$, it holds that $\sup_{h \in[H], \xi_{h} \in \Xi }\left\|\widehat{\bP}_h\left(\cdot \mid \xi_{h}\right)-\bP_h\left(\cdot \mid \xi_{h}\right)\right\|_{1} \leq \epsilon$, then we have that $\sr{\hat{\pi}^k,k} \leq  H^2 \epsilon$. In addition, if $\xi_h$ is i.i.d.,  then $\forall \delta \in(0,1)$, with probability at least $1-\delta$:
$$
\sr{\hat{\pi},K} \leq  H^2 \sqrt{\frac{2|\Xi|\log (2 H/ \delta)}{K}}.
$$
\end{proposition}
The first assumption requires the estimation error is \textit{uniformly} bounded by $\epsilon$, which is not realistic since the error typically increases with the history length $h$. The second one does not apply to the more general Markovian setting. Moreover, the straightforward extension of the proof for Exo-MAB is not valid due to the coupling/dependence of $\hat{P}_h \not\perp \hat{P}_{h'}$ for $h\neq h'$. Now we provide the cumulative regret bound of \pto for the Exo-MDP with Markovian exogenous process in Theorem \ref{thm:pto_reg}. \srscomment{What is it you are trying to say in refering to Theorem 6 in \cite{sinclair2023hindsight}? Not certain you need to include the actual regret guarantee vs just present yours}
\begin{theorem}%[Cumulative Regret Bound of PTO for 1-Markovian]
\label{thm:pto_reg}
If $\boldsymbol{\xi}$ is Markovian, then $\forall \delta \in(0,1)$, with probability at least $1-\delta$
\begin{align*}
    \rgr{\ftl,K} &\leq  4H^2|\Xi|\sqrt{2K\log(2KH|\Xi|/\delta)} + H\sqrt{KH\log(2KH|\Xi|/\delta)}. 
\end{align*}
In addition, the expected regret bound can be bounded as
\[ \bE[\rgr{\ftl,K}] \leq 4H^2|\Xi|\sqrt{2K\log(KH|\Xi|/\delta)}. \]
\end{theorem}
\paragraph{Proof sketch.}
The proof proceeds by controlling the plug-in model error at the level of the \emph{exogenous rows}. Since the next state is a deterministic push-forward of the exogenous variable given $(s_h,a_h)$,
$s_{h+1}=(f(x_h,a_h,\xi_{h+1}),\xi_{h+1})$, Lemma~\ref{lem:dp} (data-processing in TV) yields
\[
\epsilon_h^k(s_h,a_h)
=\bigl\|P_h(\cdot\mid s_h,a_h)-\widehat P_h^k(\cdot\mid s_h,a_h)\bigr\|_1
\;\le\;
\epsilon_h^k(\xi_{h})
=\bigl\|P_h(\cdot\mid \xi_{h})-\widehat P_h^k(\cdot\mid \xi_{h})\bigr\|_1,
\]
so the estimation error is \emph{policy-/action-independent}. Concentration with the exogenous count
$C_h^k(\xi):=\sum_{l=1}^{k-1}\mathbb{I}\{\xi_h^l=\xi\}$ gives
$\epsilon_h^k(\xi)\lesssim\sqrt{(2|\Xi|\,\iota)/C_h^k(\xi)}$ where $\iota=\log(2KH|\Xi|/\delta)$.
Plugging these errors into the simulation lemma and unrolling over the horizon (either the expected version, Lemma~\ref{lem:sim_exp}, or the martingale-difference version, Lemma~\ref{lem:sim_mar}) gives the per-episode suboptimality
$\sum_{h=1}^{H-1}(H-h)\,\epsilon_h^k(\cdot)$. Summing over $k$ and using the visit-sum inequality
$\sum_{k=1}^K \! 1/\sqrt{C_h^k(\xi)} \le 2\sqrt{C_h^K(\xi)}$, then summing over $\xi$ and $h$, yields the leading term
$4H^2|\Xi|\sqrt{2K\,\iota}$. To obtain a high-probability bound, we control the fluctuation between
$[P_h|\cdot|]$ and realized next-state evaluations via the MDS form in Lemma~\ref{lem:sim_mar} under the \emph{essential filtration} $\mathcal{G}_h^k:=\sigma\big((s_1^m,\boldsymbol{\xi}^m)_{m\le k-1},\,s_1^k,\,(\xi_{h'}^k)_{h'\le h-1}\big)$ generated solely by the exogenous trace. Azuma-Hoeffding plus a union bound over $(h,\xi)$ contributes the additive $H\sqrt{KH\,\iota}$ term. Taking expectations removes the martingale term, yielding the stated expected-regret bound.

The main technical challenge is the policy misalignment issue, where a direct state-action analysis fails because counts $C_h^k(s,a)$ are taken along the greedy trajectory, while the comparator uses optimal trajectories; this mismatch prevents telescoping of $\sum_k \epsilon_h^k(\tilde{s}_h^k,\tilde{a}_h^k)$. We resolve this technical challenge via two
technical novelties: (i) We replace state-action counts by exogenous-row counts $C_h^k(\xi)$ and invoke Lemma~\ref{lem:dp} so that model error becomes policy-/action-independent, eliminating any dependence on the endogenous state/action sizes and avoiding misalignment; (ii) we validate the MDS simulation lemma under Markovian $\boldsymbol{\xi}$ by working with the exogenous filtration $\mathcal{G}_h^k$, which decouples rows despite temporal dependence and enables the high-probability control.

We provide the regret bound of Optimistic Value Iteration in Proposition [] (in Appendix []?).

\subsection{Impossibility of pure exploitation under general MDP} 
%------------------------------
% Main impossibility results
%------------------------------
\begin{proposition}%[Linear regret \ftl]
\label{prop:ftl_mab_lb}
Fix any $A\ge 2$ and any gap $\Delta\in(0,\tfrac14]$. Consider Bernoulli MAB with means $\mu_1=\tfrac12+\Delta, \mu_2=\cdots=\mu_K=\tfrac12$. Run \ftl with warm-start %$L=1$
(each arm pulled once) and then act greedily. For all $K\ge A$, $\mathbb{E}[\mathrm{Regret}(K)]
\;\ge\;
\Bigl(\tfrac12-\Delta\Bigr)\!\Bigl(1-2^{-(A-1)}\Bigr)\,\Delta\,(K-A)
\;=\;\Omega(K)$.
\end{proposition}
The proof of Proposition \ref{prop:ftl_mab_lb} is deferred to Appendix [].

\srscomment{Hmm - OK I think we can talk about this tomorrow. But I think this section has some nice points that you are trying to make, but the way that it is organized makes these a little bit difficult to follow. My interpretation is that the main point is ``In Exo-MDPs, pure exploitation strategies should work, even under Markovian noise.  Moreover, these strategies in general are computationally effient for tabular settings.''

More directly aligned toward this I would do the following:
\begin{itemize}
    \item Begin with a short paragraph saying that since the only unknown in an Exo-MDP is the exogenous distribution (unaffected by actions), intuitively exploration is not needed (since the data observed is ``independent'' of the policy). We highlight this by providing algorithms in two simpler settings.
    \item Start with bandits, include a {\em brief} paragraph (potentially with a paragraph header) saying that a variant of FTL is exploration free and is regret optimal. Then emphasize that this is ``in contrast'' to the performance of FTL in {\em non} or {\em normal} MABs (where you need to do UCB or whatever).
    \item Then go to the tabular setting. I would skip the ERM discussion (only point you are trying to make is in reference to computation, that can be made just with a sentence by saying ``Note that this is in contrast to the ERM algorithm of \citet{sinclair2023hindsight} which yields similar guarantees but has computational complexity XXX.''
    \item Finish the section by emphasizing, these algorithms are fine and all, but had some serious assumptions (tabular), and next we show how to use these approaches under LFA.
\end{itemize}
}


==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

\newcommand{\tsum}{\textstyle\sum}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> parts/app_algorithm.tex <==
\section{Omitted discussion in Section \ref{sec:lfa}}
\label[appendix]{app:lfa_discussion}


\subsection{\texttt{LSVI-PE} with misspecification (approximation) error.}
\label[appendix]{app:approx_error}

\srsedit{
Here we consider the case where the function class is misspecified and the true value functions may not lie exactly in the linear span. To capture this, we introduce the notion of post–decision Bellman operators.
}
Write $x' := g(x^{a},\xi')$. For any $U_{h+1}:\mathcal{X}\times\Xi\to\mathbb{R}$,
\begin{align*}
(\mathcal{T}^{\pi} U_{h+1})(x^{a},\xi)
&:= \mathbb{E}_{\xi' \sim P_h(\cdot\mid \xi)}\!\Big[\, r\!\big(x',\pi(x',\xi'),\xi'\big)
+ U_{h+1}\!\big(\mathcal{T}^{\pi}_{h}(\xi')(x^a),\,\xi'\big) \Big],\\
(\mathcal{T} U_{h+1})(x^{a},\xi)
&:= \mathbb{E}_{\xi' \sim P_h(\cdot\mid \xi)}\!\Big[\, \max_{a'\in\mathcal{A}}
\big\{ r(x',a',\xi') + U_{h+1}\!\big(f^a(x',a'),\,\xi'\big) \big\} \Big].
\end{align*}
%\paragraph{Function class and misspecification.} 
Let $\mathcal{F}_h:=\{(x^a,\xi)\mapsto \phi(x^a)^\top w_h(\xi):\,w_h(\xi)\in\R^d\}$ be the post-decision linear class at stage $h$.

\srsedit{We then have the Bellman errors or approximation errors as follows:}

\begin{definition}[Inherent Bellman error]\label{def:IBE}
Define the (post-decision) inherent Bellman errors
\[
\varepsilon_{\mathrm{BE}}^{\pi}:=\max_{h\in[H]}\sup_{\xi\in\Xi}\ \sup_{U_{h+1}\in\mathcal{F}_{h+1}}\ \inf_{W_h\in\mathcal{F}_h}\ \sup_{x^a}\big|(T^\pi U_{h+1})(x^a,\xi)-W_h(x^a,\xi)\big|,
\]
\[
\varepsilon_{\mathrm{BE}}^{\max}:=\max_{h\in[H]}\sup_{\xi\in\Xi}\ \sup_{U_{h+1}\in\mathcal{F}_{h+1}}\ \inf_{W_h\in\mathcal{F}_h}\ \sup_{x^a}\big|(\cT U_{h+1})(x^a,\xi)-W_h(x^a,\xi)\big|.
\]
We will use $\varepsilon_{\mathrm{BE}}:=\max\{\varepsilon_{\mathrm{BE}}^{\pi^\star},\,\varepsilon_{\mathrm{BE}}^{\max}\}$.
\end{definition}

\begin{comment}
\paragraph{Algorithm (LSVI-PE).}
At episode $k$ we form empirical row-stochastic estimates $\widehat P^k(\cdot\mid\xi)$ from the first $k-1$ episodes. Going backward $h=H,\dots,1$, we compute for each $\xi$ a target vector on the anchors,
\[
y^k_h(n;\xi)=\sum_{\xi'}\widehat P^k(\xi'|\xi)\left[r\big(x_h(n),a^{n}_h(n,\xi),\xi'\big)+\phi\!\big(f^a(x_h(n),a^{n}_h(n,\xi))\big)^\top w^n_{h+1}(\xi')\right],
\]
where $a^{n}_h(n,\xi)$ is greedy w.r.t.\ the current $w^n_{h+1}$. Then solve the (anchor) least-squares system
\[
w^k_h(\xi)=\Sigma_h^{-1}\sum_{n=1}^N \phi(x^a_h(n))\,y^k_h(n;\xi).
\]
Deploy the greedy policy $\hat\pi_k$ induced by $\{w^k_h\}_{h=1}^H$ in episode $k$.
\end{comment}
% \hao{to reduce space, can we move the definition of two operators and definition 3 to appendix, and give some explanation of the $\varepsilon_{\mathrm{BE}}$ instead? We could do this if we cannot reduce space anymore}

\AgnosticRegret*
% \begin{restatable}{theorem}{AgnosticRegret}[Agnostic Regret]
% \label{thm:reg-agnostic}
% Assume Assumption~\ref{asp:anchor} holds.  Fix $\delta\in(0,1)$. Then with probability at least $1-\delta$,
% \begin{align*}
%     \mathrm{Regret}(K)\ \le\ \cO \prt{ 
% \,H\,\sqrt{K\iota}
% \;+\;
% \,|\Xi|H\Big(H+\sqrt{\tfrac{N}{\lambda_0}}\Big)\sqrt{K\iota}
% \;+\;
% \,\frac{H}{\sqrt{\lambda_0}}\,K\,\varepsilon_{\mathrm{BE}} }.
% \end{align*}
% %Here $\varepsilon_{\mathrm{BE}}$ is the inherent Bellman error from Definition~\ref{def:IBE}.
% \end{restatable}

% Now use: \AgnosticRegret*

\srsedit{Compared to the realizable case, the regret bound now includes an additional bias term, linear in $K$, that scales with the inherent Bellman error $\varepsilon_{\mathrm{BE}}$. This term is unavoidable in general agnostic settings: if $\varepsilon_{\mathrm{BE}}>0$ is fixed, even an oracle learner suffers an $O(K\varepsilon_{\mathrm{BE}})$ cumulative bias \citep{zanette2020learning}.}

\begin{comment}
\begin{remark}[Tightness and sublinearity conditions]\label{rem:tightness}
The linear-in-$K$ penalty is minimax-unavoidable in general agnostic settings: if $\varepsilon_{\mathrm{BE}}>0$ is fixed, even an oracle learner suffers an $O(K\varepsilon_{\mathrm{BE}})$ cumulative bias. Thus, sublinear regret requires either (i) realizability ($\varepsilon_{\mathrm{BE}}=0$), or (ii) a \emph{feature refinement} schedule that drives $\varepsilon_{\mathrm{BE}}=\varepsilon_{\mathrm{BE}}(k)\to 0$ sufficiently fast, or (iii) structure that shrinks the relevant \emph{on-policy} error (below).
\end{remark}
\end{comment}


\subsection{Example where Assumption \ref{asp:blt} holds}
\textbf{Models.} Consider an storage control Exo-MDP where the endogenous (pre-decision) storage state is $x_h\in[0,R_{\max}]$. 
At each stage the controller chooses an action $a_h\in\mathcal A(x_h,\xi_h)\subset\mathbb R$, which produces the post-decision storage
\[
x_h^{a}=\Pi_{[0,R_{\max}]}\big(x_h+a_h\big),
\]
where $\Pi$ denotes projection onto $[0,R_{\max}]$. 
After acting, the exogenous state evolves as $\xi_{h+1}\sim \bP(\cdot\mid \xi_h)$ and the storage evolves according to
\[
x_{h+1}=\Pi_{[0,R_{\max}]}\!\big(A(\xi_{h+1})\,x_h^{a}+b(\xi_{h+1})\big),
\]
with efficiency/retention factor $A(\xi')\in[0,1]$ and inflow/outflow $b(\xi')\in\mathbb R$. 
The next post-decision storage under policy $\pi$ is then
\[
x_{h+1}^{a}=\Pi_{[0,R_{\max}]}\!\big(x_{h+1}+\pi(x_{h+1},\xi_{h+1})\big).
\]
The one-period reward is a bounded measurable function $r_h(x_h,a_h,\xi_h)$.

\textbf{Basis, anchors, and value representation.}
Choose storage anchors $0=\rho_0<\rho_1<\cdots<\rho_N=R_{\max}$. 
Define nonnegative, nodal, partition-of-unity piecewise-linear hat functions $\{\eta_k(\rho)\}_{n=0}^N$, and set
\[
\phi(\rho)=(\eta_0(\rho),\dots,\eta_N(\rho)), \qquad \phi(\rho_n)=e_n.
\]
Thus each $\phi(\rho)$ is a convex combination of anchor vectors. 
The post-decision value is represented using storage-only features and information-dependent weights:
\[
V_{h}^{\pi,a}(x^a,\xi) \;=\; \phi(x^a)^\top\, w_h^{\pi}(\xi),
\]
where $w_h^{\pi}(\xi)\in\mathbb R^{N+1}$ and $[w_h^{\pi}(\xi)]_n=V_h^{\pi,a}(\rho_n,\xi)$. 
At the terminal time, weights encode salvage values, e.g.\ $w_H^{\pi}(\xi)=0$ or $[w_H^{\pi}(\xi)]_n=S(\rho_n,\xi)$.

Recall that Assumption \ref{asp:blt} holds if for each $h$, policy $\pi$, and exogenous realization $\xi'$, there exists a storage-feature transport matrix $M_{h}^{\pi}(\xi')\in\mathbb R^{(N+1)\times(N+1)}$ such that for all post-decision storage states $x^a\in[0,R_{\max}]$,
\[
\phi\!\Big(\Pi\big(\alpha_{h,\pi}(\xi')\,x^a+\beta_{h,\pi}(\xi')\big)\Big)\;=\;M_{h}^{\pi}(\xi')\,\phi(x^a),
\]
where $\alpha_{h,\pi}(\xi')$ and $\beta_{h,\pi}(\xi')$ are the coefficients induced by the composition of the storage dynamics and the policy’s action, followed by projection. 
Crucially, $M_{h}^{\pi}(\xi')$ does not depend on $x^a$, so the identity holds globally. 
The weights evolve linearly in expectation over $\xi'$:
\[
w_h^{\pi}(\xi) \;=\; \mathbb E_{\xi'\sim \bP(\cdot\mid \xi)}\!\big[\, M_{h}^{\pi}(\xi')^{\!\top}\, w_{h+1}^{\pi}(\xi') \,\big].
\]
This formulation is reasonable under the following conditions. 
First, the post-decision to next pre-decision mapping is affine in $r^a$, possibly followed by clipping. 
Second, the policy $\pi$ is piecewise-affine in $r$, so that the overall map to $r_{h+1}^a$ is affine with clipping. 
Third, the storage basis $\phi$ is translation-stable: for any affine map $r\mapsto \Pi(\alpha r+\beta)$ there exists a fixed sparse matrix $S_{\alpha,\beta}$ such that $\phi(\Pi(\alpha r+\beta))=S_{\alpha,\beta}\phi(r)$ for all $r$. 
Finally, since $\phi$ forms a partition of unity and clipping corresponds to convex mixing with boundary anchors, each $M_{h}^{\pi}(\xi')$ is row-stochastic or sub-stochastic, and therefore non-expansive with $\|M_{h}^{\pi}(\xi')\|_\infty\le 1$.
\begin{comment}
The exogenous state is $\xi_h$, endogenous pre-decision storage is $r_h$, and the action is $a_h$ with post-decision storage $r_h^a$. 
Dynamics are determined by $\bP$, $A(\xi')$, and $b(\xi')$, while the reward is $r_h(x_h,a_h,\xi_h)$. 
Anchors are storage breakpoints $\{\rho_k\}$ only, with basis vectors $\phi(\rho)$ depending on storage alone. 
Weight vectors are $w_h^{\pi}(\xi)\in\mathbb R^{N+1}$ for each $\xi$, storing post-decision values at anchors. 
Global closure means that there exist matrices $M_{h}^{\pi}(\xi')$ such that $\phi(\cdot)$ is transported linearly for all $r^a$, and the weights evolve according to the linear recursion given above.
\end{comment}

\subsection{When Assumption \ref{asp:nn_cone} holds}
\label{sec:when-nn-cone}

Assumption~\ref{asp:nn_cone} requires that every post-decision feature vector can be written as a nonnegative combination of a fixed set of \emph{anchor} feature vectors. This section lists common modeling choices under which the condition is automatically satisfied and gives a simple recipe to enforce it in practice. Assumption~\ref{asp:nn_cone} aligns with widely used feature constructions in ADP/RL (tabular, hat/spline, histogram, grid/ReLU bases).

\paragraph{Tabular features.}
With one-hot features, each post-decision state corresponds to a standard basis vector, which is in the conic (indeed, convex) hull of the anchor set by construction.

\paragraph{Storage with piecewise-linear (hat) features.}
Let $0=\rho_0<\rho_1<\cdots<\rho_N=R_{\max}$ be storage anchors and define nonnegative, nodal, partition-of-unity hat functions $\{\eta_n\}_{n=0}^N$.
Set $\phi(\rho)=(\eta_0(\rho),\dots,\eta_N(\rho))$ so that $\phi(\rho_n)=e_n$ and $\sum_n \eta_n(\rho)=1$ for all $\rho$.
For any post-decision level $x^a\in[0,R_{\max}]$, we have $\phi(x^a)=\sum_n \eta_n(x^a)\, \phi(\rho_n)$ with $\eta_n(x^a)\ge 0$, so $\phi(x^a)$ lies in the conic hull of the anchor features (in fact, in their convex hull).
Clipping at the bounds $0$ and $R_{\max}$ simply mixes with boundary anchors and preserves nonnegativity.

\paragraph{Histogram / indicator bases.}
If $\phi$ is formed by nonoverlapping (or softly overlapping) nonnegative basis functions that sum to at most one (e.g., bin indicators or triangular kernels), then $\phi(x^a)$ is a nonnegative combination of the anchor features obtained by placing anchors at the bin centers or knot points.

\paragraph{B-splines and ReLU tiles.}
Nonnegative partition-of-unity spline bases (e.g., linear B-splines) and grid-based ReLU “tiles” yield $\phi(x^a)$ with nonnegative entries and local support.
Choosing anchors at the knots/cell corners makes $\phi(x^a)$ a nonnegative combination of anchor feature vectors.

%\paragraph{A sufficient design recipe.}
To ensure Assumption~\ref{asp:nn_cone}:
(i) include boundary anchors so that clipping/projection maps to anchors;
(ii) use nonnegative, locally supported basis functions that form (approximate) partitions of unity over the post-decision domain;
(iii) place anchors at the basis nodes (knots, cell corners, or representative states) so that $\phi(\text{state})$ is a sparse nonnegative combination of anchor columns.
If a signed feature map is preferred (e.g., mean-centered features), a standard fix is a \emph{nonnegative lifting} $\tilde\phi = [\phi_+;\,\phi_-]$ with $\phi_+=\max\{\phi,0\}$ and $\phi_-=\max\{-\phi,0\}$; placing anchors on the lifted coordinates restores the cone property.



\subsection{When the bound $\sup_{\pi,\xi,t}\|M_h^{\pi}(\xi)\|_2\leq 1$ holds}
Recall under Assumption \ref{asp:blt_anchor} or Assumption \ref{asp:blt} that for each $(h,\pi,\xi')$ one builds a mixing matrix
\[
M_h^{\pi}(\xi') \in \mathbb{R}^{(N+1)\times(N+1)},
\]
whose $n$-th row contains the interpolation weights $\beta_{nj}(\xi',\pi)\ge 0$ (usually two nonzeros) taking the anchor $\rho_n$ to the next post-decision storage $r_{h+1}^a$ and then back onto the anchor grid. Thus each row sums to~1 (row-stochastic; sub-stochastic at the capacity boundaries when clipping pins to $\rho_0$ or $\rho_N$). We provide some sufficient conditions for $\|M_h^{\pi}(\xi')\|_2 \le 1$ below.

\emph{Lipschitz-in-storage dynamics with hat basis.}
If the continuous map $T(r)=\Pi(\alpha r+\beta)$ is $1$-Lipschitz (i.e., $|\alpha|\le 1$) and functions of $r$ are represented on a uniform grid with nodal PLC interpolation, then the discrete composition operator $\text{interpolate}\circ T$ is nonexpansive on grid values under the Euclidean norm. This operator is exactly $M_h^{\pi}(\xi')^\top$, hence $\|M_h^{\pi}(\xi')\|_2\le 1$.
Intuitively, $1$-Lipschitz maps do not increase distances between storage levels; interpolation preserves (and slightly underestimates) distances, so the induced linear map is nonexpansive.

\emph{Doubly (sub-)stochastic mixing.}
If every $M_h^{\pi}(\xi')$ is row-stochastic and column-sub-stochastic (all column sums $\le 1$), then
\[
\|M_h^{\pi}(\xi')\|_2 \;\le\;\sqrt{\|M_h^{\pi}(\xi')\|_1\,\|M_h^{\pi}(\xi')\|_{\infty}}
\;\le\;\sqrt{1\cdot 1}\;=\;1.
\]
Column-sub-stochasticity holds, for example, if the one-step map in storage is monotone and nonexpansive: $r^a\mapsto \Pi(\alpha r^a+\beta)$ with $|\alpha|\le 1$, and the basis is nodal hat (partition-of-unity) features on a uniform grid. Each anchor’s ``mass'' spreads to at most two neighbors without duplication, and clipping removes mass near the boundaries.

\emph{Decomposition into contractions.}
If the mixing matrix can be expressed as a convex combination of contractions,
\[
M_h^{\pi}(\xi') = \sum_{\ell} \gamma_\ell T_\ell, \qquad
\gamma_\ell \ge 0,\ \sum_\ell \gamma_\ell=1,\ \ \|T_\ell\|_2\le 1,
\]
then by subadditivity and convexity of the operator norm,
\(\|M_h^{\pi}(\xi')\|_2 \le 1\).
Two useful instances are: \emph{Permutation/shift structure:} when the map is a grid shift or clipping, each $T_\ell$ is a permutation (possibly composed with a boundary projector), hence $\|T_\ell\|_2=1$. \emph{Row-weighted permutations:} if $M=\sum_\ell D_\ell \Pi_\ell$ with $\Pi_\ell$ permutations and $D_\ell$ diagonal with entries in $[0,1]$, then $\|M\|_2 \le \sum_\ell \|D_\ell\|_2 \le \sum_\ell \max_i (D_\ell)_{ii}$.
  If the row-wise weights over $\ell$ sum to $\le 1$, the bound is~$\le 1$.

\emph{Doubly-stochastic special case.}
If columns also sum to $1$ (e.g., pure permutations, or measure-preserving monotone maps without clipping on a periodic grid), then $M$ is doubly stochastic and $\|M\|_2 \le 1$ with equality only if $M$ is a permutation.

Furthermore, we provide some methods to check or enforce the assumption. Empirically, one can draw a batch of $\xi'\sim Q(\cdot\mid \xi)$, build $M_h^{\pi}(\xi')$, and compute the largest singular value $\sigma_{\max}$, verifying $\max \sigma_{\max}\le 1$ (allowing numerical tolerance). 
Design-wise, one can ensure nonexpansiveness by using uniform nodal hat features (partition of unity), storage dynamics with $|\alpha|\le 1$, and capacity clipping. 
If some scenarios have $|\alpha|>1$ (expansive), increase grid resolution or add a smoothing step (row-wise convex averaging) that preserves row sums, making $M$ a contraction. 
For non-uniform grids or unusual features, ``whitening'' each local two-anchor block (normalizing columns per cell) enforces contraction while preserving row sums.

\begin{comment}
\textbf{When the bound can fail.}
If $|\alpha|>1$ so that mass from multiple anchors funnels into the same neighbors (column sums exceed~1), $\|M\|_2$ can exceed~1. 
With wide, non-nodal, or sign-changing bases (e.g., global polynomials, RBFs without partition-of-unity normalization), overlapping columns can yield $\|M\|_1>1$, breaking the bound even if rows sum to~1.
\end{comment}

Under storage-only anchors and nodal, nonnegative, partition-of-unity hat basis, and with standard storage dynamics (affine $+$ clipping) satisfying $|\alpha|\le 1$, the transport matrices $M_h^{\pi}(\xi')$ are row-stochastic and column-sub-stochastic. Hence $\sup_{\pi,\xi,h}\,\|M_h^{\pi}(\xi)\|_2 \;\le\; 1$. This can be verified numerically, and if needed enforced by smoothing or per-cell normalization without altering the PLC interpolation semantics.

\paragraph{Connections to \cite{nascimento2013optimal}.}
Under the modeling assumptions in \cite{nascimento2013optimal} the bound is justified when one implements the storage-only anchor/hat-basis scheme. \cite{nascimento2013optimal} works in post-decision form and shows that, for each information state, the value function in the scalar storage is piecewise-linear concave with breakpoints. Each period’s decision is obtained from a deterministic linear program with vector-valued control, and the algorithm maintains concavity of slopes via projection. This is exactly the setting where one uses storage-only anchors $\{\rho_n\}$ and nodal hat features. The storage dynamics between periods are affine plus clipping: the model introduces exogenous changes in storage in post-decision form, so that the next storage is an additive update (possibly with losses) followed by projection to capacity. This map is $1$-Lipschitz in the storage variable.  

With nodal, nonnegative, partition-of-unity hat functions on $\{\rho_n\}$, the push-forward and interpolation step from an anchor $\rho_n$ produces a row-stochastic mixing row (two nonzeros in one dimension). Collecting these rows defines the matrix $M_h^{\pi}(\xi)$. Because the underlying continuous map is $1$-Lipschitz and interpolation is stable, the induced discrete operator on nodal values is nonexpansive in the Euclidean norm, hence $\|M_h^{\pi}(\xi)\|_2 \le 1$. At capacity boundaries, clipping only reduces distances, so the bound continues to hold. This is consistent with the PLC/anchor structure and concavity projection used in the paper.
It should be noted that the paper does not phrase its analysis in terms of an $M$ matrix or a spectral-norm bound. Instead, it proceeds via a dynamic programming operator on slope vectors with technical conditions ensuring monotonicity, continuity, and convergence. Thus the spectral-norm assumption is an implied property of the standard discretization, rather than a stated theorem.  

In summary, for \cite{nascimento2013optimal}, with the standard storage law (additive exogenous changes with clipping) and the PLC/anchor representation, the discretization induces row-stochastic (and nonexpansive) mixing operators. Therefore it is reasonable and consistent to assume $\sup_{\pi,\xi,h}\|M_h^{\pi}(\xi)\|_2 \le 1$, even though the paper establishes convergence via slope-operator monotonicity and continuity rather than an explicit spectral-norm bound.



==> parts/app_experiments.tex <==
\section{Detailed numerical experiments}
\label[appendix]{app:exp}


\subsection{Tabular MDP}
We conduct numerical experiments using tabular Exo-MDPs, and display the model estimation error over episodes and the regret comparison between \pto and \texttt{PTO-Opt} in Figure~\ref{fig:tabular_results}.
We provide the implementation details below.
\begin{itemize}[leftmargin=*]  
  \item \textbf{Model estimation.} \pto or \lsvi estimates the model \(\widehat P_t(y'\mid y)\) from past episodes (counts per time-step) and solves backward DP using \(\widehat P_{t}\) .
  \item \textbf{Optimistic model.} At each Bellman backup the \texttt{PTO-Opt}  solves \(\max_{Q: \|Q-\widehat P\|_1\le\text{bonus}}\!\sum_{y'} Q(y')V(y')\) by mass transfer  to obtain an optimistic expectation.
  \item \textbf{Policy evaluation.} All algorithms are evaluated by exact backward induction on the true \(P_y\) to obtain stage-\(1\) value functions \(V(\cdot,\cdot,1)\).
  \item \textbf{Regret and model error.} Per episode we measure instantaneous regret as
  \(\sum_{x,y}\big(V^\star_{x,y,1}-V^{\pi}_{x,y,1}\big)\) and report cumulative regret \(\sum_{k\le K}\) (averaged across runs). Model error is measured by the average Frobenius norm \(\frac{1}{T}\sum_{t}\| \widehat P_t-P_y\|_F\).
  %\item \textbf{Visualization.} Curves (mean \(\pm\) std) are smoothed with a moving-average window of size 20 and saved as \texttt{pto\_regret\_curve.png}.
\end{itemize}

\paragraph{Baseline methods.}
We compare the \pto to \texttt{PTO-Opt} (Section \ref{sec:pto-opt}) that solves a constrained \(\ell_1\)- subproblem for optimistic model with confidence radius
  \(\text{bonus}=c\sqrt{2Y\log(KY/0.01)/N_{t,y}}\) (default \(c=0.3\)).
\begin{figure}[bh]
    \centering
    % left
    \begin{subfigure}{1\linewidth}
        \centering
        \includegraphics[width=0.64\linewidth]{iclr2026/figs/regret_curve_c0.3.pdf} 
    \end{subfigure}
    \caption{Comparison between \pto and \texttt{PTO-Opt}. }
    \label{fig:tabular_results}
    \vspace{-4ex}
\end{figure}

\begin{figure}[th]
    \centering
    % left
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{iclr2026/figs/lsvi_pe_results_ep100_T6_R10_K10_c0.5.pdf}
        \caption{$H=6$}
        \label{fig:lsvi_results_h6}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{iclr2026/figs/lsvi_pe_results_ep100_T8_R10_K10_c0.5.pdf}
        \caption{$H=8$ }
        \label{fig:lsvi_results_h8}
    \end{subfigure}
    \hfill
    % right
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{iclr2026/figs/lsvi_pe_results_ep100_T10_R10_K10_c0.5.pdf}
        \caption{$H=10$}
        \label{fig:lsvi_results_h10}
    \end{subfigure}
    \caption{Comparison of \lsvi and \texttt{LSVI-Opt} across three different time horizon lengths. 
    }
    \label{fig:lsvi_results}
    \vspace{-2ex}
\end{figure}

\subsection{Storage control}
We display the model estimation error over episodes and the regret comparison between \lsvi and \texttt{LSVI-Opt} in Figure~\ref{fig:lsvi_results} across three Exo-MDPs with different horizon lengths. Across $H\in\{6,8,10\}$, \lsvi consistently outperforms \texttt{LSVI-Opt} in cumulative regret.

We provide the pseudo-code of \lsvi for storage control in Algorithm \ref{alg:lsvi-pe-storage}.

\paragraph{Baseline method.} \texttt{LSVI-Opt} differs from \lsvi in Line 12 of
Algorithm \ref{alg:lsvi-pe-storage}. Specifically, \texttt{LSVI-Opt} computes the optimistic target 
\[ y^k_h(n)\gets \displaystyle\sum_{\xi'\in\Xi} \tilde{P}^k_h(\xi'\mid\xi)\!\cdot\!\max_{a'\in[-a_{\max},a_{\max}]}\Big\{
r\!\big(g(\rho_n,\xi'),a',\xi'\big)+\phi\!\big(f^a(g(\rho_n,\xi'),a')\big)^\top w^k_{h+1}(\xi')\Big\},  \]
where $\tilde{P}^k_h$ is the optimistic model obtained by solving the $\ell_1$ constrained subproblem around $\hat{P}^k_h$ with  confidence radius \(\text{bonus}=c\sqrt{2Y\log(KY/0.01)/N_{t,y}}\) (default \(c=0.5\)).

\paragraph{Detailed setup.}
We numerically analyze a storage control problem with continuous endogenous state space $\X=[0,C]$, discrete exogenous state space $\Xi=[Y]$, and continuous action space $\A=[-a_{max}, a_{max}]$. $\X$ is discretized by $N$ anchors. The default parameters are $C=10$, $Y=10$, $a_{max}=2$, $N=10$, and $K=100$ epsiodes. Three time horizon lengths $H\in \{6,8,10\}$ are evaluated for comparison. The exogenous variable is the discrete power price with the following transition rules applied: a 70~$\%$ probability exists of either remaining in the original state or transitioning to an adjacent state, with the remaining 30~$\%$ assigned to uniform selection among all feasible states.


\paragraph{Computational efficiency.} The major computational overhead of Algorithm \ref{alg:lsvi-pe-storage} is to solve the optimal action for a given state $s^k_h$ at each time-step $h$
$$ \hat\pi^k_h(x^k_h,\xi^k_h)=\arg\max_{a\in[-a_{\max},a_{\max}]}\ \big\{r(x^k_h,a,\xi^k_h)+\phi\!\big(f^a(x^k_h,a)\big)^\top w^k_{h+1}(\xi^k_h)\big\}. $$
We emphasize this step is computationally efficient via anchor enumeration due to the LP structure of the subproblem.

\begin{algorithm}
\caption{\texttt{LSVI-PE} for storage control}
\label{alg:lsvi-pe-storage}
\begin{algorithmic}[1]
\Require Horizon $H$; capacity $C$; anchors $\rho_n=\frac{n-1}{N-1}C,\ n=1...N$; hat features $\phi:[0,C]\!\to\!\mathbb{R}^N$ with $\phi(\rho_n)=e_n$
\Require Action set $\mathcal{A}=[-a_{\max},a_{\max}]$; efficiencies $\eta^+,\eta^->0$; leakage $\alpha\in(0,1]$
\Require Reward $r(s,a,\xi)=\xi a-\alpha_c|a|-\beta_h s$; post-decision $f^a(s,a)=\mathrm{clip}\!\big(s+\eta^+a^+-\tfrac{1}{\eta^-}a^-,\,0,\,C\big)$; pre-decision update $g(s^a,\xi')=\alpha s^a$
\Require Price codebook $\Xi=\{\zeta_1,\dots,\zeta_R\}$; dataset of $k$ price trajectories $\{\xi_h^\ell\}_{\ell=1,h=1}^{k,H}$ with $\xi_h^\ell\in\Xi$
\State \textbf{Update $\hat{P}^k_h(\cdot\mid \xi)$}: for each $(h,\xi)$,
\[
\hat{P}^k_h(\xi'\mid \xi)=
\begin{cases}
\frac{N^k_h(\xi,\xi')}{\sum_z N^k_h(\xi,z)}, & \sum_z N^k_h(\xi,z)>0\\
\frac{1}{R}, & \text{otherwise (unvisited row)}
\end{cases}
\]
where $N^k_h(\xi,\xi')=\sum_{\ell=1}^k \mathbf{1}\{\xi_h^\ell=\xi,\ \xi_{h+1}^\ell=\xi'\}$.
\State \textbf{Backward Value Iteration:}
\For{$h=H$ down to $1$}
  \For{each $\xi\in\Xi$}
    \State \Comment{Design at post-decision anchors (identity under hat basis)}
    \State $\Phi_h \gets [\phi(\rho_1),\ldots,\phi(\rho_n)]$;\ \ $a_h \gets \Phi_h\Phi_h^\top$ \Comment{$\Phi_h=I_K,\ a_h=I_K$}
    \State $b^k_h(\xi)\gets \mathbf{0}\in\mathbb{R}^K$
    \For{$n=1$ to $N$}
      \If{$h=H$}
        \State $y^k_h(n)\gets 0$
      \Else
        \State $y^k_h(n)\gets \displaystyle\sum_{\xi'\in\Xi} \hat{P}^k_h(\xi'\mid\xi)\!\cdot\!\max_{a'\in[-a_{\max},a_{\max}]}\Big\{
r\!\big(g(\rho_n,\xi'),a',\xi'\big)+\phi\!\big(f^a(g(\rho_n,\xi'),a')\big)^\top w^k_{h+1}(\xi')\Big\}$
        \State \Comment{Inner $\max$ is 1-D LP (piecewise linear); solve via  breakpoint enumeration}
      \EndIf
      \State $b^k_h(\xi)\gets b^k_h(\xi)+\phi(\rho_n)\,y^k_h(n)$ \Comment{writes $y^k_h(n)$ into entry $k$}
    \EndFor
    \State $w^k_h(\xi)\gets \Sigma_h^{-1}b^k_h(\xi)$ \Comment{with $\Sigma_h=I_N$: $w^k_h(\xi)=[y^k_h(1),\ldots,y^k_h(N)]^\top$}
  \EndFor
\EndFor
\State \textbf{Output:}
\State $\hat V^{k,a}_h(x^a,\xi)=\phi(x^a)^\top w^k_h(\xi)$,\quad for all $(s^a,\xi,h)$
%\State $\hat\pi^k_h(s,\xi)=\arg\max_{a\in[-a_{\max},a_{\max}]}\ \big\{r(s,a,\xi)+\phi\!\big(f^a(s,a)\big)^\top w^k_h(\xi)\big\}$,\quad for all $(s,\xi,h)$
\State \textbf{return} $\hat V^{k,a}_h$ 
\end{algorithmic}
\end{algorithm}






==> parts/app_preliminary.tex <==
\section{Omitted discussion in Section \ref{sec:pre}}
\label[appendix]{app:preliminary}

%\srscomment{finished a draft}

\paragraph{$m$-Markovian exogenous process.} We note that our framework extends to exogenous processes with finite memory.  Specifically, we assume that the exogenous state follows a $m$-Markov model: at time $h$, the augmented state includes the endogenous component $x_h$ together with the last $m$ exogenous states,
\[s_h = \bigl(x_h, \xi_{h-m}, \ldots, \xi_h\bigr).\]
The next exogenous state $\xi_{h+1}$ is drawn from a conditional distribution that depends only on the most recent $k$ exogenous states:
\[
\xi_{h+1} \sim \bP\!\left(\cdot \,\bigm|\, \xi_{h-m},\ldots,\xi_h\right).
\]
This formulation strictly generalizes the i.i.d.\ and first-order Markov settings while retaining a compact representation that captures temporal correlations in the exogenous sequence.

\paragraph{Known functions dynamics and reward functions $f$ and $g$.}  Our model assumes that the endogenous dynamics $f$ and the reward function $r$ are known and deterministic given the exogenous state. While this assumption is more restrictive than the fully general unknown MDP model typically studied in the RL literature, it is well-motivated in many operations research domains.  Indeed, inventory control, pricing, scheduling, and resource allocation problems are often modeled with deterministic system dynamics where the only uncertainty arises from exogenous randomness~\citep{powell2022reinforcement}.  This assumption also aligns with the practice of simulator-based design, widely adopted in queueing and inventory control studies (e.g.,~\cite{madeka2022deep,alvo2023neural,che2024differentiable}).

\subsection{Example applications of Exo-MDP}
\label[appendix]{app:exo_mdp_examples}

We close out with a brief discussion of models in operations research that can be represented as Exo-MDPs. We have introduced the storage control in Section \ref{sec:exp-tab}. See~\citep{powell2022reinforcement,sinclair2023adaptive} for a more exhaustive list.


\paragraph{Inventory control.}  
In classical inventory models, the endogenous state $x_h$ is the on-hand inventory level, while the exogenous state $\xi_h$ is the demand realization at time $h$~\citep{madeka2022deep}. Actions $a_h$ correspond to order quantities. The system dynamics are deterministic given demand, e.g. the newsvendor dynamics \ $x_{h+1} = f(x_h,a_h,\xi_{h+1}) = \max\{x_h+a_h-\xi_{h+1},0\}$. The reward depends on sales revenue and holding or stockout costs, $r(x_h,a_h,\xi_h)$. The only randomness arises from the exogenous demand process, making this a canonical instance of an Exo-MDP.

\paragraph{Cloud resource allocation.}  
In cloud computing and service systems, the endogenous state $x_h$ may represent the allocation of resources (e.g., virtual machines, CPU quotas, or bandwidth) across job requests~\citep{sinclair2023hindsight}. The exogenous state $\xi_h$ captures job arrivals at time $h$, which evolve independently of the resource allocation policy. Actions $a_h$ correspond to  scheduling decisions, and the reward reflects performance metrics such as throughput or delay penalties. The exogenous job-arrival process drives all stochasticity, while the system dynamics (queue updates, resource usage) are deterministic given arrivals.




==> parts/app_proofs.tex <==
\section{Proofs of regret bounds in Section \ref{sec:wm}}
\label[appendix]{app:wm}

\subsection{Exo-Bandits}

\FTLBandits*

To show the result we start with the following lemma.

\begin{lemma}[Maxima of sub-Gaussian random variables]
\label{lem:max}
Let $X_1, \ldots, X_n$ be independent $\sigma^2$-sub-Gaussian random variables. Then
\begin{equation*}
    \mathbb{E}\left[\max _{1 \leq i \leq n} X_i\right] \leq \sqrt{2 \sigma^2 \log n}
\end{equation*}
and, for every $t>0$,
\begin{equation*}
    \mathbb{P}\left\{\max _{1 \leq i \leq n} X_i \geq \sqrt{2 \sigma^2(\log n+t)}\right\} \leq e^{-t},
\end{equation*}
or equivalently 
\begin{equation*}
    \mathbb{P}\left\{\max _{1 \leq i \leq n} X_i \geq \sqrt{2 \sigma^2 \log(n/\delta)}\right\} \leq \delta,
\end{equation*}
\end{lemma}
\begin{proof}
The first part is quite standard: by Jensen's inequality, monotonicity of exp, and $\sigma^2$-subgaussianity, we have, for every $\lambda>0$,
$$
e^{\lambda \mathbb{E}\left[\max_{1 \leq i \leq n} X_i\right]} \leq \mathbb{E} e^{\lambda \max _{1 \leq i \leq n} X_i}=\max _{1 \leq i \leq n} \mathbb{E} e^{\lambda X_i} \leq \sum_{i=1}^n \mathbb{E} e^{\lambda X_i} \leq n e^{\frac{\sigma^2 \lambda^2}{2}}
$$
so, taking logarithms and reorganizing, we have
$$
\mathbb{E}\left[\max _{1 \leq i \leq n} X_i\right] \leq \frac{1}{\lambda} \ln n+\frac{\lambda \sigma^2}{2} .
$$
Choosing $\lambda:=\sqrt{\frac{2 \ln n}{\sigma^2}}$ proves the first inequality. Turning to the second inequality, let $u:=\sqrt{2 \sigma^2(\log n+t)}$. We have
$$
\mathbb{P}\left\{\max _{1 \leq i \leq n} X_i \geq u\right\}=\mathbb{P}\left\{\exists i, X_i \geq u\right\} \leq \sum_{i=1}^n \mathbb{P}\left\{X_i \geq u\right\} \leq n e^{-\frac{u^2}{2 \sigma^2}}=e^{-t}
$$
the last equality recalling our setting of $u$. 
\end{proof}
%The upper bound on the expectation of maxima  is not a high probability bound (independent of $\delta$).
Now we provide the proof of Proposition \ref{prop:ftl_mab}.
\begin{proof}
Observe that the empirical mean is unbiased for each arm at each round, 
    \begin{align*}
        \sr{\ftl,k} &= \mu^{\star} - \bE[\mu_{a_k} ] = \max_{a}\bE[\mu_a - \mu_{a_k} ]=\max_{a}\bE[\hat{\mu}_a(k) - \mu_{a_k} ] \leq \bE[\max_{a}\hat{\mu}_a(k) - \mu_{a_k} ] \\
        &= \bE[\hat{\mu}_{a_k}(k) - \mu_{a_k} ] \\
        &\leq \bE[\max_{a\in[A]}\hat{\mu}_{a}(k) - \mu_{a} ] \\
        &\leq \sqrt{2\sigma^2\log A/(k-1)},
    \end{align*}
where the last inequality is due to Lemma \ref{lem:max}. Therefore, we have
\[ \rgr{\ftl,K} = \sum_{k=1}^K \sr{\ftl,k} \leq \sum_{t=2}^K\sqrt{2\sigma^2\log A/(k-1)} \leq 2\sigma\sqrt{(K-1)\log A}. \]
\end{proof}

\begin{comment}
\begin{remark}
The following statement is wrong
\[ \bE[\hat{\mu}_{a_k}(k)]= \bE[\mu_{a_k}]. \]
In fact, we have 
\[\bE[\hat{\mu}_{a_k}(k)] \ge \mu^{\star}>\bE[\mu_{a_k}].\]
On the other hand, since $\hat{\mu}_{k}(k)>\hat{\mu}_{a}(k),\forall a\neq k$ conditioned on that $a_k=k$, we have 
\[  \bE[\hat{\mu}_{a_k}(k)|a_h=k]=\bE[\hat{\mu}_{k}(k)|a_h=k]\ge \bE[\hat{\mu}_{1}(k)|a_k=k]=\mu_1. \]
The last step may be wrong, but at least we can get
\[  \bE[\hat{\mu}_{a_k}(k)|a_k=k]=\bE[\hat{\mu}_{k}(k)|a_h=k]\ge \mu_k. \]
Therefore,
\[ \bE[\hat{\mu}_{a_k}(k)] = \bE[\bE[\hat{\mu}_{a_k}(k)|a_k]] = \sum_a\bP(a_k=a)\bE[\hat{\mu}_{a_k}(k)|a_k=a] \ge \sum_a\bP(a_k=a)\mu_a =\bE[\mu_{a_k}]. \]
\end{remark}
\begin{remark}
We can obtain the finer upper bound for the Gaussian bandit.  
\end{remark}
\end{comment}
\begin{comment}
\paragraph{Failure under bandit feedback}
Under the bandit feedback, the empirical mean for each arm depends on the visiting count 
\[ \hat{\mu}_{a}(k):= 1/C_{a}(k)\sum_{s=1}^{k-1}\bI\cbrk{A_s=a}r(a,\xi_s). \]
Importantly, the agent cannot observe $\xi_k$.

The following proof is wrong.
\begin{align*}
    \bE[\rgr{\ftl,K}] &= \bE[\sum_{k=1}^K \sr{\ftl,k}] = \bE[\sum_{k=1}^K \mu^{\star}-\mu_{a_k}]\\
    &= \bE[\sum_{h=1}^T \underbrace{\mu^{\star}-\hat{\mu}_1(k)}_{(a)}+\underbrace{\hat{\mu}_1(k)-\hat{\mu}_{a_k}(k)}_{(b)}+\underbrace{\hat{\mu}_{a_k}(k)-\mu_{a_k}}_{(c)}]\\
    &= \bE[\sum_{k=1}^K \underbrace{\hat{\mu}_1(k)-\hat{\mu}_{a_k}(k)}_{(b)}+\underbrace{\hat{\mu}_{a_k}(k)-\mu_{a_k}}_{(c)}] \\
    &\leq \bE[\sum_{k=1}^K \underbrace{\hat{\mu}_{a_k}(k)-\mu_{a_k}}_{(c)}]\\
    &\leq \bE[\sum_{k=1}^K \cO(\sqrt{\frac{1}{C_k(a_k)}})] \\
    &\leq \cO(\sqrt{AK})
\end{align*}
Step $(a)$ uses the statement that given the visiting count, the empirical mean maintained for each arm at each round is unbiased
\[ \bE[ \hat{\mu}_{a}(k)|C_{a}(k)]=1/C_a(k)\bE[ \sum_{s=1}^{k-1}\bI\cbrk{A_s=a}r(a,\xi_s)|C_{a}(k)]=\mu_a, \]
implying 
\[  \bE[ \hat{\mu}_{a}(k)]=\bE[\bE[ \hat{\mu}_{a}(k)|C_{a}(k)]]=\mu_a. \]
However, the first claim is NOT true by noting that 
\begin{align*}
    \bE[ \hat{\mu}_{a}(k)|C_{a}(k)=c]&=\frac{1}{c}\bE\brk{ \sum_{s=1}^{k-1}\bI\cbrk{A_s=a}r(a,\xi_s)|\sum_{s=1}^{k-1}\bI\cbrk{A_s=a}=c} \\
    &\neq \frac{1}{c}\bE\brk{ \sum_{s=1}^{k-1}\bI\cbrk{A_s=a}|\sum_{s=1}^{k-1}\bI\cbrk{A_s=a}=c}\bE[r(a,\xi_s)]=\mu_a.
\end{align*}
For instance, consider a two armed bandit with $\mu_1>\mu_2$. We will show that for some $c>0$ and $t>1$ the statement does not hold.  Note that 
\ftl chooses $A_1=1$ and $A_2=2$. Let $c=1$ and $t\ge3$. Conditioned on the event $\cbrk{C_1(k+1)=1}$, we have 
\begin{align*}
\cbrk{C_1(k+1)=1}&=\cbrk{\sum_{s=3}^{k}\bI\cbrk{A_s=1}=0}=\cbrk{A_s=2,\forall3\leq s\leq k}\\
&=\cbrk{\hat{\mu}_1(s)<\hat{\mu}_2(s),\forall 3\leq s \leq k}\\
&= \cbrk{r(1,\xi_{1})<\frac{1}{s-2}\sum_{s'=2}^{s-1}r(2,\xi_{s'}),\forall 3\leq s \leq k} \\
&=\cbrk{r(1,\xi_{1})<r(2,\xi_{2})}\cap\cbrk{r(1,\xi_1)<\frac{1}{2}(r(2,\xi_{2})+r(2,\xi_{3}))}\cap\cdots.
\end{align*}
Let $k=3$. Since $\cbrk{C_1(3+1)=1}=\cbrk{r(1,\xi_{1})<r(2,\xi_{2})}$, we have
\begin{align*}
\bE\brk{\hat{\mu}_1(4)|C_1(4)=1}=\bE\brk{r(1,\xi_{1})|C_1(4)=1}=\bE\brk{r(1,\xi_{1})|r(1,\xi_{1})<r(2,\xi_{2})}.
\end{align*}
Let $X_1=r(1,\xi_1)$, $X_2= r(2,\xi_2)$ be two independent r.v.s. Consider the discrete bandit
\begin{align*}
\bE\brk{\hat{\mu}_1(4)|C_1(4)=1}=\bE\brk{X_1|X_1<X_2}&=\sum_{x_2} P_{X_2}(x_2)\sum_{x_1<x_2}P_{X_1}(x_1)x_1 \\
&< \sum_{x_2} P_{X_2}(x_2)\sum_{x_1}P_{X_1}(x_1)x_1  =\bE[x_1]=\mu_1.
\end{align*}
Similar result holds for the continuous bandit 
\begin{align*}
\bE\brk{\hat{\mu}_1(4)|C_1(4)=1}=\bE\brk{X_1|X_1<X_2}&=\int_{x_2\in\bR} p_{X_2}(x_2)\int_{x_1<x_2}p_{X_1}(x_1)x_1dx_1dx_2 \\
&< \int_{x_2\in\bR} p_{X_2}(x_2)\int_{x_1\in\bR}p_{X_1}(x_1)x_1dx_1dx_2  =\bE[x_1]=\mu_1.
\end{align*}
\begin{remark}
The key insight is that the visiting count $C_h$ is dependent on the algorithm, and thus is coupled with the historical observations $r(A_s,\xi_s)_{s\in[k-1]}$ since the algorithm chooses actions based on the particular history. Therefore, given different visiting count, the empirical mean is biased. In the example above, the small visiting count favors underestimated realization for arm 1.    
\end{remark}
\begin{remark}
    Full information does NOT have such problem. $C_k(a)=k-1$ $\forall a,t$.
\end{remark}
\end{comment}

\subsection{Tabular Exo-MDP}

\ERMExoMDP*
\begin{proof}
Observe that $V_1^\pi\left(s_1, \boldsymbol{\xi}^k\right)$ are iid r.v.s, each of which has mean $V_1^\pi\left(s_1\right)$. Using Hoeffding's inequality and a union bound over all policies shows that the event
$$
\mathcal{E}=\left\{\forall \pi \in \Pi:\left|V_1^\pi\left(s_1\right)-\overline{\mathbb{E}}\left[V_1^\pi\left(s_1\right)\right]\right| \leq \sqrt{\frac{H^2 \log (2|\Pi| / \delta)}{2 K}}\right\}
$$
occurs with probability at least $1-\delta$. Under $\mathcal{E}$ we then have
$$
\begin{aligned}
\sr{\ftl,K} &= V_1^{\pi^{\star}}\left(s_1\right)-V_1^{\hat{\pi}^k}\left(s_1\right) \\
& =V_1^{\pi^{\star}}\left(s_1\right)-\overline{\mathbb{E}}\left[V_1^{\pi^{\star}}\left(s_1, \boldsymbol{\xi}\right)\right]+\overline{\mathbb{E}}\left[V_1^{\pi^{\star}}\left(s_1, \boldsymbol{\xi}\right)\right]-\overline{\mathbb{E}}\left[V_1^{\hat{\pi}^k}\left(s_1, \boldsymbol{\xi}\right)\right]\\
&+\overline{\mathbb{E}}\left[V_1^{\hat{\pi}^k}\left(s_1, \boldsymbol{\xi}\right)\right]-V_1^{\hat{\pi}^k}\left(s_1\right) \\
& \leq 2 \sqrt{\frac{H^2 \log (2|\Pi| / \delta)}{2 K}}.
\end{aligned}
$$
\end{proof}

\FTLExoMDP*
\begin{proof}
It holds that 
    \begin{align*}
        \bE[\sr{ \ftl,K}] &= V_1^{\pi^{\star}}\left(s_1\right)-\bE[V_1^{\hat{\pi}^k}\left(s_1\right)] 
        = \max_{\pi} \bE[\overline{\mathbb{E}}\left[V_1^\pi\left(s_1,\boldsymbol{\xi}\right)\right]] - \bE[V_1^{\hat{\pi}^k}\left(s_1\right)] \\
        &\leq  \bE[\max_{\pi}\overline{\mathbb{E}}\left[V_1^\pi\left(s_1,\boldsymbol{\xi}\right)\right]] - \bE[V_1^{\hat{\pi}^k}\left(s_1\right)] \\
        &= \bE[ \widetilde{V}_1^{\hat{\pi}^k}(s_1) - V_1^{\hat{\pi}^k}\left(s_1\right) ] \\
        &\leq \bE [\max_{\pi} \widetilde{V}_1^{\pi}(s_1)-V_1^{\pi}\left(s_1\right) ] \\
        &\leq \sqrt{\frac{ H^2 \log |\Pi| }{K}},
    \end{align*}
    where the last inequality is due to Lemma \ref{lem:max}.
\end{proof}



\subsection{Proof of Theorem \ref{thm:pto_reg}}
\begin{lemma}[Data processing inequality, TV distance]
\label{lem:dp}
Let $\mu,\nu$ be two probability measures on a discrete set $X$ and $f:X\rightarrow Y$ be a mapping. Let $f_{\#,\mu}$ and $f_{\#,\nu}$ be  the resulting push-forward measures on the space $Y$. Then
\[ \norm{f_{\#,\mu}-f_{\#,\nu}}_1 \leq \norm{\mu-\nu}_1. \]
\begin{proof}
    \begin{align*}
        \norm{f_{\#,\mu}-f_{\#,\nu}}_1&=\sum_{y\in Y}|f_{\#,\mu}(y)-f_{\#,\nu}(y)|=\sum_{y\in Y}|\mu(f^{-1}(y))-\nu(f^{-1}(y))| \\
        & =\sum_{y\in Y}|\sum_{x\in f^{-1}(y)}\mu(x)-\sum_{x\in f^{-1}(y)}\nu(x)| \\
        &\leq  \sum_{y\in Y}\sum_{x\in f^{-1}(y)}|\mu(x)-\nu(x)| \leq \sum_{x\in X}|\mu(x)-\nu(x)|=\norm{\mu-\nu}_1,
    \end{align*}
    where the second inequality is due to the triangle inequality.
\end{proof}
\end{lemma}
\subsubsection{Proof using expected simulation lemma}
\begin{lemma}[Simulation lemma, expected version]
\label{lem:sim_exp}
Let $\cM=(P,r)$ and $\cM=(P',r)$. Define
\[ \epsilon_h(s,a):=\norm{P_h(s,a) - P'_h(s,a)}_1 \leq \sqrt{\frac{2S\log}{C_h(s,a)}}.\]
For any fixed policy $\pi$ and $s_1\sim \rho$,
\[ |V^{\pi,\cM} - V^{\pi,\cM'}| \leq \bE\brk{\sum_{h=1}^{H-1}(H-h)\epsilon_h(s_h,a_h)|\pi,P,\rho}. \]
It also holds that for any $s_1$
\[ |V^{\pi,\cM}(s_1) - V^{\pi,\cM'}(s_1)| \leq \bE\brk{\sum_{h=1}^{H-1}(H-h)\epsilon_h(s_h,a_h)|\pi,P,s_1}. \]
\end{lemma}
\begin{proof}
For two different MDPs, their values are defined for the same initial distribution $\rho(s_1)$
    \begin{align*}
        |V^{\pi,\cM} - V^{\pi,\cM'}|&=|\bE[V_1^{\pi,\cM}(s_1)] - \bE[V_1^{\pi,\cM'}(s_1)]|\\
        &=|\bE[r_1(s_1,\pi_1(s_1))+[P_1 V_2^{\pi,\cM}](s_1,\pi_1(s_1))-r_1(s_1,\pi_1(s_1))-[P'_1 V_2^{\pi,\cM'}](s_1,\pi_1(s_1))]| \\
        &=|\rho[P_1 (V_2^{\pi,\cM}-V_2^{\pi,\cM'})](s_1,\pi_1(s_1))+\rho[(P_1-P'_1) V_2^{\pi,\cM'}](s_1,\pi_1(s_1))| \\
        &\leq |\bE[V_2^{\pi,\cM}(s_2)-V_2^{\pi,\cM'}(s_2)|s_2\sim \rho P_1^{\pi}]|+(H-1)\cdot\bE[\epsilon_1(s_1,a_1)|s_1\sim \rho,a_1=\pi_1(s_1)] \\
        & = |V_2^{\pi,\cM}-V_2^{\pi,\cM'}|+(H-1)\cdot\bE[\epsilon_1(s_1,a_1)|s_1\sim \rho,a_1=\pi_1(s_1)]\\
        &\leq |V_3^{\pi,\cM}-V_3^{\pi,\cM'}]|+\bE[(H-1)\epsilon_1(s_1,a_1)+(H-2)\epsilon_1(s_2,a_2)|\pi,P,\rho]\\
        &\cdots \\
        &\leq \bE\brk{\sum_{h=1}^{H-1}(H-h)\epsilon_h(s_h,a_h)|\pi,P,\rho}.
    \end{align*}
\end{proof}
Note that the expectation is taken w.r.t. 
\[ s_1\sim\rho_1, \cdots, a_h=\pi_h(s_h),s_{h+1}\sim P_h(s_h,a_h),\cdots.\]
The policy $\pi$ and transitions $P,P'$ are considered fixed, which implies that $\epsilon_h(s,a)$ is NOT random for fixed $(s,a)$.

For $k\in[K]$, $h\in[H]$, define the filtration as 
\[  \mathcal{F}^k_h:=\sigma((s^m_h,a^m_h)_{m\in[k-1],h\in[H]},(s^k_{h'},a^k_{h'})_{h'\in[h-1]}). \]
The policy $\hat{\pi}^k$ is measurable w.r.t. $\cF^n_0$, hence
\[ \hat{\pi}^k\perp \boldsymbol{\xi}^k |\cF_k,\]
but
\[  \hat{\pi}^k \not\perp (s^k_{h},a^k_{h})_{h \in [H]} |\cF_k. \]
Observe that
$$
\begin{aligned}
V_1^{\star}\left(s_1\right)-V_1^{\hat{\pi}^k}\left(s_1\right)& = V_1^{\star}\left(s_1\right)-\widehat{V}_1^{k,\pi^{\star}}\left(s_1\right)+\widehat{V}_1^{k,\pi^{\star}}\left(s_1\right)-\widehat{V}^k_1\left(s_1\right)+\widehat{V}^k_1\left(s_1\right)-V_1^{\hat{\pi}^k}\left(s_1\right) \\
& \leq \left|V_1^{\pi^{\star}}\left(s_1\right)-\widehat{V}_1^{k,\pi^{\star}}\left(s_1\right)\right| + \left|V_1^{\hat{\pi}^k}\left(s_1\right)-\widehat{V}_1^{k,\hat{\pi}^k}\left(s_1\right)\right|.
\end{aligned}
$$
Define 
\begin{align*}
   \epsilon^k_h(\xi_{h-1})&:= \norm{P_h(\xi_h\in\cdot|\xi_{h-1})-\widehat{P}^k_h(\xi_h\in\cdot|\xi_{h-1})}_1 \\
   C^k_h(\xi)&:=\sum_{m=1}^{k-1}\bI\cbrk{\xi^k_h=\xi},
\end{align*}
where $C^k_h(\xi)$ is defined by $\cF^k_0$. 

\paragraph{Key observation} Since $s_{h+1}=(f(x_h,a_h,\xi_{h}),\xi_{h})$ is a mapping of $\xi_h$ given $x_h$ and $a_h$, \textbf{for any (deterministic) policy/action sequence} and any $s_h$, it follows from Lemma \ref{lem:dp}
\[ \epsilon^k_h(s_h,a_h):= \norm{P_h(s_{h+1}\in\cdot|s_h,a_h)-\widehat{P}^k_h(s_{h+1}\in\cdot|s_h,a_h)}_1 \leq \epsilon^k_h(\xi_{h-1}) \leq \cO(\sqrt{\frac{|\Xi|\iota}{C^k_h(\xi_{h-1})}}),\]
which bounds the model estimation error by a \textit{policy/action-independent} error term. This will lead to tighter regret bound than directly bounding the model error 
\[ \epsilon^k_h(s_h,a_h)\leq \cO(\sqrt{\frac{|S|\iota}{C^k_h(s_h,a_h)}}). \]
Furthermore, we will see that the use of Exo-state $\xi_{h-1}$ overcomes the \textit{misalignment} issue since the sequence $\boldsymbol{\xi}^{k-1}$ is always $\cF^k$-measurable. Note that $C^k,\hat{P}^k,\hat{\pi}^k$ are all $\cF^k$-measurable, then $\epsilon^k(\cdot)$ is also $\cF^k$-measurable. 

\paragraph{The failure of using state-action count.}
Denote by $(s^k_h,a^k_h)_{h\in[T]}$ and $(\tilde{s}^k_h,\tilde{a}^k_h)_{h\in[T]}$ the sequence generated by $(\hat{\pi}^k,P)$ and $(\pi^{\star},P)$ at the $n$-th episode.  In particular, 
\[  \tilde{s}^k_1=s^k_1=x^k_1, \tilde{a}^k_1=\pi^{\star}_1(s^k_1),\tilde{s}^k_{2}=(f(\tilde{s}^k_1,\tilde{a}^k_1,\xi^k_1),\xi^k_1),\cdots, \tilde{s}^k_{h+1}=(f(\tilde{s}^k_h,\tilde{a}^k_h,\xi^k_h),\xi^k_h),\cdots    \]
Note that $(\tilde{s}^k_h,\tilde{a}^k_h)_{h\in[H]}$ is fixed conditional on $\boldsymbol{\xi}^k$, so its randomness only comes from $\boldsymbol{\xi}^k$. We bound the \textbf{random} regret as
\begin{align*}
    \sum_{k=1}^K V^{\star}_1-V^{\hat{\pi}^k}_1 &\leq \sum_{k=1}^K V_1^{\star}-\widehat{V}_1^{k,\pi^{\star}}+\widehat{V}^k_1-V_1^{\hat{\pi}^k} \leq \sum_{k=1}^K\abs{V_1^{\pi^{\star}}-\widehat{V}_1^{k,\pi^{\star}}} + \sum_{k=1}^K\abs{V_1^{\hat{\pi}^k}-\widehat{V}^{k,\hat{\pi}^k}_1}\\
    &\leq \sum_{h=1}^{H-1}(H-h)\sum_{k=1}^K\bE\brk{ \epsilon^k_h(\tilde{s}^k_h,\tilde{a}^k_h)|\cF_k} + \sum_{h=1}^{H-1}(H-h)\sum_{k=1}^K\bE\brk{\epsilon^k_h(s^k_h,a^k_h)|\cF_k} \\
    &\leq  \sum_{h=1}^{H-1}(H-h)\bE\brk{\sum_{k=1}^K \sqrt{\frac{2S\iota}{C^k_h(\tilde{s}^k_h,\tilde{a}^k_h)}}|\cF_k} + \sum_{h=1}^{H-1}(H-h)\bE\brk{\sqrt{\frac{2S\iota}{C^k_h(s^k_h,a^k_h)}}|\cF_k},
\end{align*}
where the third inequality is due to Lemma \ref{lem:sim_exp} and the last inequality is due to Lemma
\ref{lem:dp}. However, the key is that the visiting count
\[  C^k_h(s,a) = \sum_{m=1}^{k-1} \bI\cbrk{(s^m_h,a^m_h)=(s,a)} \]
is defined by $\cF^k$ generated by $(\hat{\pi},P)$. Although we can bound the second term via standard proof, we cannot obtain an upper bound on the first term. Specifically,
\begin{align*}
   \sum_{k=1}^K \sqrt{\frac{2S\iota}{C^k_h(\tilde{s}^k_h,\tilde{a}^k_h)}} &= \sum_{k=1}^K \sum_{s,a}\bI\cbrk{(\tilde{s}^k_h,\tilde{a}^k_h)=(s,a)}\sqrt{\frac{2S\iota}{C^k_h(\tilde{s}^k_h,\tilde{a}^k_h)}}\\
   &= \sum_{s,a} \sum_{k=1}^K\bI\cbrk{(\tilde{s}^k_h,\tilde{a}^k_h)=(s,a)}\sqrt{\frac{2S\iota}{C^k_h(s,a)}} \\
   &\neq \sum_{s,a} \sum_{c=1}^{C^k_h(s,a)}\sqrt{\frac{2S\iota}{c}}.
\end{align*}
The last inequality is due to the fact that $C^k_h(s,a)$ does not increase by 1 if $(\tilde{s}^k_h,\tilde{a}^k_h)=(s,a)$ since $C^k_h$ counts based on $\cF^k$ or $(s^k_h,a^k_h)$.

\paragraph{The solution: bounding via exogenous state count.}
Using Lemma \ref{lem:sim_exp} we can get 
\begin{align*}
    \sum_{k=1}^K V^{\star}_1-V^{\hat{\pi}^k}_1 &\leq \sum_{k=1}^K V_1^{\star}-\widehat{V}_1^{k,\pi^{\star}}+\widehat{V}^k_1-V_1^{\hat{\pi}^k} \leq \sum_{k=1}^K\abs{\widehat{V}_1^{k,\pi^{\star}}-V_1^{\star}} + \sum_{k=1}^K\abs{\widehat{V}^{k,\hat{\pi}^k}_1-V_1^{\hat{\pi}^k}}\\
    &\leq \sum_{h=1}^{H-1}(H-h)\sum_{k=1}^K\bE\brk{\epsilon^k_h(\tilde{s}^k_h,\tilde{a}^k_h)|\cF_k} + \sum_{h=1}^{H-1}(H-h)\sum_{k=1}^K\bE\brk{\epsilon^k_h(s^k_h,a^k_h)|\cF_k} \\
    &\leq  2\sum_{h=1}^{H-1}(H-h)\sum_{k=1}^K\bE\brk{\sqrt{\frac{2|\Xi|\log(KH/\delta)}{C^k_h(\xi^k_{h-1})}}|\cF_k},
\end{align*}
where the expectation in the second line is taken w.r.t. the $(\tilde{s}^k_h,\tilde{a}^k_h)_{h\in[H]}\sim P^{\pi^{\star}}$ and $(s^k_h,a^k_h)_{h\in[H]} \sim P^{\hat{\pi}^k}$.
Taking expectation on both sides, we can get 
\begin{align*}
    \bE\brk{\sum_{k=1}^K V^{\star}_1-V^{\hat{\pi}^k}_1} &\leq 2\sum_{h=1}^{H-1}(H-h)\bE\brk{\sum_{k=1}^K\sqrt{\frac{2|\Xi|\log(KH/\delta)}{C^k_h(\xi^k_{h-1})}}} \leq 4H^2|\Xi|\sqrt{2N\log(KH/\delta)}.
\end{align*}

\begin{comment}
\paragraph{Distribution-dependent worst-case bound?}
Define
\[  c^k_h(\xi):=\sqrt{2|\Xi|\iota}/C_h^k(\xi) =\sqrt{2|\Xi|\iota}/\sqrt{\sum_{m=1}^{k-1} \bI\cbrk{\xi^m_h=\xi}}.    \]
Given the marginal distribution of $\xi^k_{h-1}$, we want to obtain an upper bound on $\bE[c^k_h(\xi^k_{h-1})]$. Since $c^k_h$ is independent of $\xi^k$, we have
\begin{align*}
    \bE[c^k_h(\xi^k_{h-1})] &= \bE[\sum_{\xi} \bI\cbrk{\xi^k_{h-1}=\xi}c^k_h(\xi^k_{h-1})] = \bE[\sum_{\xi} \bI\cbrk{\xi^k_{h-1}=\xi}c^k_h(\xi)] = \sum_{\xi}\bE[ \bI\cbrk{\xi^k_{h-1}=\xi}]\bE[c^k_{h}(\xi)] \\
    &= \sum_{\xi} \bP_h\prt{\xi^k_{h-1}=\xi}\bE[c^k_{h}(\xi)],
\end{align*}
where $\bP_h\prt{\xi^k_{h-1}=\cdot}$ is the marginal distribution of $\xi^k_{h-1}$. Note that $\xi^k_{h-1} \sim \bP_h\prt{\xi_{h-1}=\cdot}$ IID, hence 
$$\bI\cbrk{\xi^m_{h-1}=\xi}\sim \text{Ber}(\bP_h(\xi)) \Longrightarrow C_h^k(\xi)\sim \text{Bin}(k-1,\bP_h(\xi)).$$ 
We could obtain a \textbf{lower bound} on $\bE[c^k_h(\xi)]$ by Jensen's inequality
\[ \bE[c^k_h(\xi)]= \sqrt{2|\Xi|\iota}\bE[\frac{1}{\sqrt{C_h^k(\xi)}}] \ge \sqrt{2|\Xi|\iota}/\sqrt{\bE[C_h^k(\xi)]}=\sqrt{2|\Xi|\iota}/\sqrt{(k-1)\bP_h(\xi)}. \]
Then
\[  \bE\brk{\sum_{k=1}^K c_h^k(\xi^k_{h-1})}\ge \sum_{\xi}\bP_h(\xi)\sum_{k=1}^K\sqrt{2|\Xi|\iota}/\sqrt{(k-1)\bP_h(\xi)}=\sqrt{2|\Xi|\iota}\sum_{\xi}\sqrt{\bP_h(\xi)}\Theta(\sqrt{K})\in\sqrt{2|\Xi|K\iota}[1,\sqrt{|\Xi|}].  \]
However, we need an upper bound on $\bE[c^k_h(\xi)]$ to bound the regret as
\begin{align*}
    \sum_{\xi} \bP_h\prt{\xi}\sum_{c=1}^{k-1}\frac{1}{\sqrt{c}} {k-1 \choose c} (\bP_h(\xi))^c(1-\bP_h(\xi))^{k-1-c} \leq  \cO(\sqrt{\frac{|\Xi|}{k-1}})?
\end{align*}
\end{comment}

\subsubsection{Proof via MDS simulation lemma}
\begin{lemma}[Simulation lemma, martingale difference]
\label{lem:sim_mar}
Let $\cM=(P,r)$ and $\cM'=(P',r)$. Fix an arbitrary policy $\pi$. Define
\begin{align*}
    \epsilon_h&:=\norm{P_h(s_h,\pi_h(s_h)) - P'_h(s_h,\pi_h(s_h))}_1 \leq \sqrt{\frac{2S\log}{C_h(s_h,\pi_h(s_h))}}\\
    e_h&:= [P_h |V_{h+1}^{\pi,\cM}-V_{h+1}^{\pi,\cM'}|](s_h,\pi_h(s_h)) - |V_{h+1}^{\pi,\cM}-V_{h+1}^{\pi,\cM'}|(s_{h+1}),
\end{align*}
where $e_h$ is a martingale difference sequence w.r.t. the filtration $\mathcal{H}_h:=\sigma(s_1,\pi_1(s_1),\cdots,s_{h-1},\pi_{h-1}(s_{h-1}))$. 
Then
    \[ |V^{\pi,\cM}(s_1) - V^{\pi,\cM'}(s_1)| \leq \sum_{h=1}^{H-1} (e_h+(H-h)\epsilon_h). \]
\end{lemma}
Lemma \ref{lem:sim_mar} bounds a deterministic term by the sum of two random variables.
\begin{proof}
    \begin{align*}
        |V_1^{\pi,\cM}(s_1) - V_1^{\pi,\cM'}(s_1)| &= |r_1(s_1,\pi_1(s_1))+[P_1 V_2^{\pi,\cM}](s_1,\pi_1(s_1))-r_1(s_1,\pi_1(s_1))-[P'_1 V_2^{\pi,\cM'}](s_1,\pi_1(s_1))| \\
        &=|[P_1 (V_2^{\pi,\cM}-V_2^{\pi,\cM'})](s_1,\pi_1(s_1))+[(P_1-P'_1) V_2^{\pi,\cM'}](s_1,\pi_1(s_1))| \\
        &\leq [P_1 |V_2^{\pi,\cM}-V_2^{\pi,\cM'}|](s_1,\pi_1(s_1))+|[(P_1-P'_1) V_2^{\pi,\cM'}](s_1,\pi_1(s_1))|\\
        &=|V_2^{\pi,\cM}-V_2^{\pi,\cM'}|(s_2)+e_1+|[(P_1-P'_1) V_2^{\pi,\cM'}](s_1,\pi_1(s_1))| \\
        &\leq |V_2^{\pi,\cM}-V_2^{\pi,\cM'}|(s_2)+e_1+\epsilon_1\cdot(H-1)\\
        &\leq |V_3^{\pi,\cM}-V_3^{\pi,\cM'}|(s_3)+e_2+\epsilon_2\cdot(H-2)+e_1+\epsilon_1\cdot(H-1)\\
        &\leq \cdots \\
        &\leq |V_h^{\pi,\cM}-V_h^{\pi,\cM'}|(s_h)+\sum_{h=1}^{H-1}(e_h+(H-h)\epsilon_h)\\
        &=\sum_{h=1}^{H-1}(e_h+(H-h)\epsilon_h).
    \end{align*}
\end{proof}
Define
\begin{align*}
    \epsilon^k_h(s_h,a_h)&:=\norm{P_h(s_h,a_h) - \hat{P}^k_h(s_h,a_h)}_1 \leq \sqrt{\frac{2S\iota}{C^k_h(s_h,a_h)}}\\
    e^k_h(s_h,a_h|\pi)&:= [P_h |V_{h+1}^{\pi}-\hat{V}_{h+1}^{k,\pi}|](s_h,a_h) - |V_{h+1}^{\pi}-\hat{V}_{h+1}^{k,\pi}|(s_{h+1}),
\end{align*}
where $e^k_h$ is a martingale difference sequence that depends on $\pi$ through $\hat{V}_{h+1}^{k,\pi}$. Recall that $(s^k_h,a^k_h)_{h\in[H]}$ and $(\tilde{s}^k_h,\tilde{a}^k_h)_{h\in[H]}$ are the sequence generated by $(\hat{\pi}^k,P)$ and $(\pi^{\star},P)$ at the $k-$th episode, which satisfy $\tilde{s}^k_h=s^k_1=x^k_1$.
Using Lemma \ref{lem:sim_mar} we can get 
\begin{align*}
    \sum_{k=1}^K V^{\star}_1-V^{\hat{\pi}^k}_1 &\leq  \sum_{k=1}^K \abs{V_1^{\pi^{\star}}\left(s_1\right)-\widehat{V}_1^{n,\pi^{\star}}\left(s_1\right)} + \abs{V_1^{\hat{\pi}}\left(s_1\right)-\widehat{V}_1^{n,\hat{\pi}}\left(s_1\right)} \\
    &\leq \sum_{h=1}^{H-1} \sum_{k=1}^K e^k_h(\tilde{s}^k_h,\tilde{a}^k_h|\pi^{\star})+(H-h)\epsilon^k_h(\tilde{s}^k_h,\tilde{a}^k_h)  + \sum_{h=1}^{H-1}\sum_{k=1}^K e^k_h(s^k_h,a^k_h|\hat{\pi}^k)+(H-h)\epsilon^k_h(s^k_h,a^k_h) 
\end{align*}
The key observation is to verify MDS by considering the essential filtration  $\sigma((\boldsymbol{\xi}^k)_{n})$ instead of the full (standard) filtration $\sigma((s^k_h,a^k_h)_{k,h})$.  Formally, we define the essential filtration ($s^k_1=x^k_1$)
\[ \mathcal{G}^k_h:=\sigma((s^m_1,\boldsymbol{\xi}^m)_{m\in[k-1]},s^k_1,(\xi^k_{h'})_{h'\in[h-1]}), \] 
which is only generated by the exogenous process. This is different from the full filtration
\[  \mathcal{F}^k_h:=\sigma((s^m_h,a^m_h)_{m\in[k-1],h\in[H]},(s^k_{h'},a^k_{h'})_{h'\in[h-1]},s^k_h). \]
For any $k$ and $h$, we can recover/simulate $(\tilde{s}^k_{h'},\tilde{a}^k_{h'})_{h'\leq t}$ from $s^k_1$, $\pi^{\star}$ and $\xi^k_{h-1}$ as follows
\[ \tilde{s}^k_{h'}=(\tilde{x}^k_{h'},\xi^k_{h'-1}),\tilde{a}^k_{h'}=\pi^{\star}_{h'}(\tilde{s}^k_{h'}),\tilde{x}^k_{h'+1}=f(\tilde{x}^k_{h'},\tilde{a}^k_{h'},\xi^k_{h'}), \]
which implies that $(\tilde{s}^k_{h'},\tilde{a}^k_{h'})_{h'\leq t}$ is measurable w.r.t. $\mathcal{G}^k_{h}$. Furthermore, $\hat{P}^k_{\Xi}$ is measurable w.r.t. $\mathcal{G}^k$ implies $\hat{V}^{k,\pi^{\star}}$ is measurable w.r.t. $\mathcal{G}^k$. Then 
\[   e^k_h(\tilde{s}^k_h,\tilde{a}^k_h|\pi^{\star}) =  [P_h |V_{h+1}^{\pi^{\star}}-\hat{V}_{h+1}^{k,\pi^{\star}}|](\tilde{s}^k_h,\tilde{a}^k_h) - |V_{h+1}^{\pi^{\star}}-\hat{V}_{h+1}^{k,\pi^{\star}}|(\tilde{s}^k_{h+1}) \]
is an MDS w.r.t. $\mathcal{G}^k_h$ since
\begin{align*}
    \bE\brk{e^k_h(\tilde{s}^k_h,\tilde{a}^k_h|\pi^{\star})|\mathcal{G}^k_h} &= \bE\brk{[P_h |V_{h+1}^{\pi^{\star}}-\hat{V}_{h+1}^{k,\pi^{\star}}|](\tilde{s}^k_h,\tilde{a}^k_h) - |V_{h+1}^{\pi^{\star}}-\hat{V}_{h+1}^{k,\pi^{\star}}|(\tilde{s}^k_{h+1})|\mathcal{G}^k_h} \\
    &= [P_h |V_{h+1}^{\pi^{\star}}-\hat{V}_{h+1}^{k,\pi^{\star}}|](\tilde{s}^k_h,\tilde{a}^k_h)-[P_h |V_{h+1}^{\pi^{\star}}-\hat{V}_{h+1}^{k,\pi^{\star}}|](\tilde{s}^k_h,\tilde{a}^k_h)\\
    &=0,
\end{align*}
where the second equality is due to that the only non-measurable variable is $\tilde{s}^k_{h+1}$, and $e^k_h(\tilde{s}^k_h,\tilde{a}^k_h|\pi^{\star})\in\mathcal{G}^k_{h+1}$ since $\tilde{s}^k_{h+1}$ is measurable w.r.t. $\mathcal{G}^k_{h+1}$. 

Since $\hat{\pi}^k$ is measurable w.r.t. $\mathcal{G}^k$, $\hat{V}^{k,\hat{\pi}^k}$ and $(s^k_{h'},a^k_{h'})_{h'\leq t}$ are measurable w.r.t. $\mathcal{G}^k_{h}$. Then 
\begin{align*}
    \bE\brk{e^k_h(s^k_h,a^k_h|\hat{\pi}^k)|\mathcal{G}^k_h} &= \bE\brk{[P_h |V_{h+1}^{\hat{\pi}^k}-\hat{V}_{h+1}^{k,\hat{\pi}^k}|](s^k_h,a^k_h) - |V_{h+1}^{\hat{\pi}^k}-\hat{V}_{h+1}^{k,\hat{\pi}^k}|(s^k_{h+1})|\mathcal{G}^k_h} \\
    &= [P_h |V_{h+1}^{\hat{\pi}^k}-\hat{V}_{h+1}^{k,\hat{\pi}^k}|](s^k_h,a^k_h)-[P_h |V_{h+1}^{\hat{\pi}^k}-\hat{V}_{h+1}^{k,\hat{\pi}^k}|](s^k_h,a^k_h)\\
    &=0,
\end{align*}
and $e^k_h(s^k_h,a^k_h|\hat{\pi}^k)$ is measurable w.r.t. $\mathcal{G}^k_{h+1}$. Thus $e^k_h(s^k_h,a^k_h|\hat{\pi}^k)$ is also an MDS w.r.t $\mathcal{G}^k_{h}$. Using the Azuma-Hoeffding inequality, we obtain w.p. $1-\delta'$
\begin{align*}
    \sum_{h=1}^{H-1} \sum_{k=1}^K e^k_h(\tilde{s}^k_h,\tilde{a}^k_h|\pi^{\star})+e^k_h(s^k_h,a^k_h|\hat{\pi}^k) \leq \cO(H\sqrt{KH\log1/\delta'}).
\end{align*}

We can bound the error terms as
\begin{align*}
    \sum_{h=1}^{H-1}(H-h) \sum_{k=1}^K \epsilon^k_h(\tilde{s}^k_h,\tilde{a}^k_h)+\epsilon^k_h(s^k_h,a^k_h) 
    &\leq  2\sum_{h=1}^{H-1}(H-h) \sum_{k=1}^K \sqrt{\frac{2|\Xi|\log(KH/\delta)}{C^k_h(\xi^k_h)}} \\
    &\leq 4H^2|\Xi|\sqrt{2N\log(KH/\delta)}.
\end{align*}

\begin{remark}
    We cannot obtain a bound on the expected regret that is independent of $\delta$ as the full information MAB setting since 
    \[ V^{*,\cM}= \max_{\pi}V^{\pi,\cM} \neq  \max_{\pi}\bE[V^{\pi,\widehat{\cM}}] \leq  \bE[\max_{\pi}V^{\pi,\widehat{\cM}}]=\bE[V^{\hat{\pi},\widehat{\cM}}]. \]
\end{remark}

\begin{remark}
    We may obtain a tighter regret bound of $\cO(H\sqrt{|\Xi|KH\iota})$ by a finer analysis.
\end{remark}

\begin{remark}
    The simulation lemma MDS leads to a high prob. regret bound, while the simulation lemma expected version leads to a expected regret bound. They are the same order, but the latter one is weaker.
\end{remark}

\subsection{Proofs of impossibility results}
\label[appendix]{app:impossibility_proof}

\begin{definition}[Pure-Exploitation Greedy (PEG) after a finite warm-start]\label{def:PEG}
Fix an integer $L\ge 1$ (not growing with $K$). \emph{Warm-start:} pull each arm exactly $L$ times (in any order). \emph{Greedy phase:} for all subsequent rounds $K>AL$, play
\[
a_k \in \arg\max_{a\in[K]} \widehat{\mu}_a(k),
\]
where $\widehat{\mu}_a(k)$ is the empirical mean of arm $a$ over the learner's own past pulls of $a$. Ties are broken by any deterministic rule that is independent of future rewards.
\end{definition}

\begin{lemma}[Monotonicity barrier]\label{lem:barrier}
Consider PEG. Suppose at the start of the greedy phase there exist arms $i,j$ with $\widehat{\mu}_i(KL)=0$ and $\widehat{\mu}_j(KL)>0$. Then PEG never pulls arm $i$ again.
\end{lemma}


\begin{proof}
At any time $t\ge KL$, the empirical mean of arm $i$ remains exactly $0$ unless $i$ is pulled; conversely, any arm with at least one observed success retains an empirical mean $>0$ forever, because the count of successes for that arm can never drop to zero. Since PEG selects an arm with maximal empirical mean and $\widehat{\mu}_j(k)\ge \widehat{\mu}_j(KL)>0>\widehat{\mu}_i(k)$ for all $t\ge KL$, arm $i$ is never selected.
\end{proof}

\begin{theorem}[Linear regret for $K$-armed PEG with $L=1$]\label{thm:Karms_L1}
Fix any $K\ge 2$ and any gap $\Delta\in(0,\tfrac14]$. Consider Bernoulli arms with means
\[
\mu_1=\tfrac12+\Delta,\qquad \mu_2=\cdots=\mu_K=\tfrac12.
\]
Run PEG with warm-start $L=1$ (each arm pulled once) and then act greedily. For all $T\ge K$,
\[
\mathbb{E}[\mathrm{Regret}(T)]
\;\ge\;
\Bigl(\tfrac12-\Delta\Bigr)\!\Bigl(1-2^{-(K-1)}\Bigr)\,\Delta\,(T-K)
\;=\;\Omega(T).
\]
\end{theorem}

\begin{proof}
Let $X_{a,1}\in\{0,1\}$ be the first Bernoulli sample from arm $a$. Consider the warm-start event
\[
E:=\{X_{1,1}=0\}\;\cap\;\Bigl\{\exists\,b\in\{2,\dots,K\}\!:\;X_{b,1}=1\Bigr\}.
\]
Independence gives
\[
\mathbb{P}(E)=(1-\mu_1)\Bigl(1-\prod_{b=2}^K(1-\mu_b)\Bigr)
=\Bigl(\tfrac12-\Delta\Bigr)\Bigl(1-(\tfrac12)^{K-1}\Bigr).
\]
On $E$, after the $K$-round warm-start we have $\widehat{\mu}_1(K)=0$ and (at least) one suboptimal arm $b$ with $\widehat{\mu}_b(K)=1$. By Lemma~\ref{lem:barrier}, PEG never pulls arm $1$ again. Hence from round $K{+}1$ onward PEG plays a suboptimal arm every round, incurring per-round regret $\mu_1-\max_{a\neq1}\mu_a=\Delta$. Therefore,
\[
\mathrm{Regret}(k)\;\ge\;\Delta\,(T-K)\quad\text{on }E,
\]
and taking expectations yields the stated lower bound.
\end{proof}

\begin{theorem}[Linear regret for any fixed warm-start $L$]\label{thm:Karms_Lgeneral}
Fix $K\ge2$, any integer $L\ge1$ that does not grow with $T$, and any $\Delta\in(0,\tfrac14]$. Consider the same Bernoulli instance as in Theorem~\ref{thm:Karms_L1}. If PEG is run with warm-start size $L$ and then acts greedily, then for all $T\ge KL$,
\[
\mathbb{E}[\mathrm{Regret}(k)]
\;\ge\;
\underbrace{\Bigl(\tfrac12-\Delta\Bigr)^{\!L}\!\Bigl(1-\bigl(1-2^{-L}\bigr)^{K-1}\Bigr)}_{\text{a positive constant independent of $T$}}
\cdot \Delta\,(T-KL)
\;=\;\Omega(k).
\]
\end{theorem}

\begin{proof}
Let $S_{a,L}$ be the number of successes observed from arm $a$ during the $L$ warm-start pulls of that arm. Consider
\[
E_L:=\{S_{1,L}=0\}\;\cap\;\Bigl\{\exists\,b\in\{2,\dots,K\}\!:\;S_{b,L}=L\Bigr\}.
\]
By independence across arms during the warm-start,
\[
\mathbb{P}(S_{1,L}=0)=(1-\mu_1)^L=\bigl(\tfrac12-\Delta\bigr)^L,\qquad
\mathbb{P}(S_{b,L}=L)=\mu_b^L=(\tfrac12)^L,
\]
and therefore
\[
\mathbb{P}(E_L)=\bigl(\tfrac12-\Delta\bigr)^L\!\left(1-\bigl(1-2^{-L}\bigr)^{K-1}\right).
\]
On $E_L$, after the $KL$-round warm-start we have $\widehat{\mu}_1(KL)=0$ and at least one suboptimal arm $b$ with $\widehat{\mu}_b(KL)=1$. By Lemma~\ref{lem:barrier}, PEG never returns to arm $1$; consequently it plays a suboptimal arm in every round $t>KL$, suffering per-round regret $\Delta$. Taking expectations yields the claimed bound.
\end{proof}

\begin{corollary}[Any finite exploration budget]\label{cor:anyfinite}
Let an algorithm perform any deterministic, data-independent exploration schedule of finite length $N<\infty$ (not growing with $T$), after which it always selects an arm with maximal current empirical mean (deterministic tie-breaking independent of future rewards). Then there exists a Bernoulli $K$-armed instance on which the algorithm has $\mathbb{E}[\mathrm{Regret}(k)]=\Omega(k)$.
\end{corollary}

\begin{proof}
Map the schedule to some $L_a\ge 1$ pulls per arm $a$ during the exploration phase, with $\sum_a L_a=N$. Choose means as in Theorem~\ref{thm:Karms_L1} and define the event that the optimal arm produces only zeros in its $L_1$ pulls while at least one suboptimal arm produces only ones in its $L_b$ pulls. This event has strictly positive probability $\prod$-factor bounded away from $0$ (independent of $T$). Conditioned on this event, the post-exploration empirical means create a strict separation (optimal arm at $0$, a suboptimal arm at $1$), and Lemma~\ref{lem:barrier} applies verbatim to force perpetual suboptimal play thereafter, yielding linear regret in $T$.
\end{proof}

\begin{remark}[Beyond Bernoulli, bounded rewards]
The same conclusion holds for any rewards supported on $[0,1]$ when there exists a gap $\Delta=\mu^\star-\max_{a\neq a^\star}>0$. By Hoeffding's inequality, for any fixed $L$ there are constants $p_1,p_2>0$ (depending on $L$ and the arm means) such that with probability at least $p_1$ the optimal arm's warm-start average is $\le \mu^\star-\tfrac{\Delta}{2}$ and with probability at least $p_2$ some suboptimal arm's warm-start average is $\ge \mu^\star-\tfrac{\Delta}{4}$. The intersection has constant probability $p_1p_2>0$, producing a strict empirical mean misranking after the warm-start and thus linear regret by Lemma~\ref{lem:barrier}.
\end{remark}

\section{Proofs of regret bounds in Section \ref{sec:lfa}}
\label[appendix]{app:lfa}
\begin{comment}
We define the Bellman operators for the post-decision state framework:
\begin{align}
    [\mathcal{H}^{\pi} V^a ](x^a,\xi) &:= \mathbb{E}_{\xi' \sim P_h(\cdot|\xi)}[ r(x',\pi(x',\xi'),\xi') + V^a(f^a(x',\pi(x',\xi')),\xi') | x^a,\xi] \\
    [\mathcal{H} V^a ](x^a,\xi) &:= \mathbb{E}_{\xi' \sim P_h(\cdot|\xi)}[ \max_{a'} ( r(x',a',\xi') + V^a(f^a(x',a'),\xi') ) | x^a,\xi]
\end{align}
where $x' = g(x^a, \xi')$ is the next pre-decision state.
\end{comment}
\subsection{Proof of Theorem \ref{thm:reg_anchor}}
Define $\delta^k_h(\pi):=(V^{k,\pi}_h-V^{\pi}_h)(s^k_h)$. We have
\begin{align*}
    \delta^k_h(\pi)&=(V^{k,\pi}_h-V^{\pi}_h)(s^k_h) = (V^{k,\pi}_h-V^{\pi}_h)(x^k_h,\xi^k_{h-1}) \\
    &=r(x^k_h,\pi,\xi^k_{h-1})+V_h^{k,\pi,a}(f^a(x^k_h,\pi),\xi^k_{h-1}) - r(x^k_h,\pi,\xi^k_{h-1}) - V_h^{\pi,a}(f^a(x^k_h,\pi),\xi^k_{h-1}) \\
    &=\phi(f^a(x^k_h,\pi))^\top ( w^{k,\pi}_h(\xi^k_{h-1}) - w^{\pi}_h(\xi^k_{h-1}) ) \\
    &=:\phi(x^{k,\pi}_h)^\top ( w^{k,\pi}_h(\xi^k_{h-1}) - w^{\pi}_h(\xi^k_{h-1}) ) \\
    &=\phi(x^{k,\pi}_h)^\top \Sigma_h^{-1}\Phi_h (\bv^{k,\pi}_h(\xi^k_{h-1}) - \bv^{\pi}_h(\xi^k_{h-1})),
\end{align*}
where 
\begin{align*}
    \bv^{k,\pi}_h(\xi^k_{h-1},n)&=\sum_{\xi^k_{h}} \hat{P}^k_h(\xi^k_{h}|\xi^k_{h-1}) 
    \brk{r(g(x_h^a(n),\xi^k_{h}),\pi,\xi^k_{h}) + \phi(f^a(g(x_h^a(n),\xi^k_{h}),\pi))^\top w^{k,\pi}_{h+1}(\xi^k_{h})} \\
    &=:\sum_{\xi^k_{h}} \hat{P}^k_h(\xi^k_{h}|\xi^k_{h-1}) 
    \brk{r(x^k_{h+1}(n),\pi,\xi^k_{h}) + \phi(f^a(x^k_{h+1}(n),\pi))^\top w^{k,\pi}_{h+1}(\xi^k_{h})} \\
    \bv^{\pi}_h(\xi^k_{h-1},n)&=\sum_{\xi^k_{h}} P_h(\xi^k_{h}|\xi^k_{h-1}) 
    \brk{r(g(x_h^a(n),\xi^k_{h}),\pi,\xi^k_{h}) + \phi(f^a(g(x_h^a(n),\xi^k_{h}),\pi))^\top w^{\pi}_{h+1}(\xi^k_{h})} \\
    &=:\sum_{\xi^k_{h}} P_h(\xi^k_{h}|\xi^k_{h-1}) 
    \brk{r(x^k_{h+1}(n),\pi,\xi^k_{h}) + \phi(f^a(x^k_{h+1}(n),\pi))^\top w^{\pi}_{h+1}(\xi^k_{h})}.
\end{align*}
Note that we denote $x^{k,\pi}_h:=f^a(x^k_h,\pi(x^k_h,\xi^k_{h-1}))$ which implicitly depends on $\xi^k_{h-1}$ and $x^k_{h+1}(n):=g(x_h^a(n),\xi^k_{h}))$ which implicitly depends on $\xi^k_{h}$. We have 
\begin{align*}
    \delta^k_h(\pi)&= \phi(x^{k,\pi}_h)^\top \Sigma_h^{-1}\Phi_h^\top (\bv^{k,\pi}_h(\xi^k_{h-1}) - \bv^{\pi}_h(\xi^k_{h-1})) \\
    &= \phi(x^{k,\pi}_h)^\top \Sigma_h^{-1} \sum_{k} \phi(x_h^a(n)) \brk{ \sum_{\xi^k_{h}} (\hat{P}^k_h(\xi^k_{h}|\xi^k_{h-1})-P_h(\xi^k_{h}|\xi^k_{h-1})) r(x^k_{h+1}(n),\pi,\xi^k_{h})  } \\
    &+\phi(x^{k,\pi}_h)^\top \Sigma_h^{-1} \sum_{k} \phi(x_h^a(n))\cdot\\
    &\brk{ \sum_{\xi^k_{h}} \hat{P}^k_h(\xi^k_{h}|\xi^k_{h-1}) \phi(f^a(x^k_{h+1}(n),\pi))^\top w^{k,\pi}_{h+1}(\xi^k_{h}) - P_h(\xi^k_{h}|\xi^k_{h-1}) \phi(f^a(x^k_{h+1}(n),\pi))^\top w^{\pi}_{h+1}(\xi^k_{h}) }.
\end{align*}
Under Assumption \ref{asp:blt_anchor}, we have
\begin{align*}
    w^{k,\pi}_h(\xi^k_{h-1}) &= \Sigma_h^{-1}\Phi_h \sum_{\xi^k_{h}} \hat{P}^k_h(\xi^k_{h}|\xi^k_{h-1}) 
    \brk{r(g(x_h^a(\cdot),\xi^k_{h}),\pi,\xi^k_{h}) + \phi(f^a(g(x_h^a(\cdot),\xi^k_{h}),\pi))^\top w^{k,\pi}_{h+1}(\xi^k_{h})} \\
    &=\Sigma_h^{-1}\Phi_h [\hat{P}^k_h \textbf{r}](\xi^k_{h-1}) + \Sigma_h^{-1}\sum_k \phi_h(k) \sum_{\xi^k_{h}} \hat{P}^k_h(\xi^k_{h}|\xi^k_{h-1}) (M^{\pi}_h(\xi^k_{h}) \phi_h(k))^\top w^{k,\pi}_{h+1}(\xi^k_{h}) \\
    &= \Sigma_h^{-1}\Phi_h [\hat{P}^k_h \textbf{r}](\xi^k_{h-1}) +\Sigma_h^{-1}\sum_k \phi_h(k)\phi_h(k)^\top \sum_{\xi^k_{h}} \hat{P}^k_h(\xi^k_{h}|\xi^k_{h-1}) (M^{\pi}_h(\xi^k_{h}))^\top w^{k,\pi}_{h+1}(\xi^k_{h}) \\
    &= \Sigma_h^{-1}\Phi_h [\hat{P}^k_h \textbf{r}](\xi^k_{h-1}) + \sum_{\xi^k_{h}} \hat{P}^k_h(\xi^k_{h}|\xi^k_{h-1}) (M^{\pi}_h(\xi^k_{h}))^\top w^{k,\pi}_{h+1}(\xi^k_{h}) \\
    &= \Sigma_h^{-1}\Phi_h [\hat{P}^k_h \textbf{r}](\xi^k_{h-1}) +  [\hat{P}^k_h ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}).
\end{align*}
Similarly, we can get 
\begin{align*}
    w^{\pi}_h(\xi^k_{h-1}) = \Sigma_h^{-1}\Phi_h [P_h \textbf{r}](\xi^k_{h-1}) +  [P_h ((M^{\pi}_h)^\top w^{\pi}_{h+1})](\xi^k_{h-1}).
\end{align*}
Thus
\begin{align*}
    &w^{k,\pi}_h-w^{\pi}_h = \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) + [\hat{P}^k_h ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}) - [P_h ((M^{\pi}_h)^\top w^{\pi}_{h+1})](\xi^k_{h-1}) \\
    &= \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) + [(\hat{P}^k_h-P_h) ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}) + [P_h ((M^{\pi}_h)^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1}))](\xi^k_{h-1}) \\
    &=\Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) + [(\hat{P}^k_h-P_h) ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}) \\
    &+ [P_h ((M^{\pi}_h)^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1}))](\xi^k_{h-1})-(M^{\pi}_h(\xi^k_{h}))^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}) + (M^{\pi}_h(\xi^k_{h}))^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}) \\
    &=:\epsilon^k_h(\pi)+e^k_h(\pi)+ (M^{\pi}_h(\xi^k_{h}))^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}),
\end{align*}
where we define 
\begin{align*}
    e^k_h(\pi)&:= [P_h ((M^{\pi}_h)^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1}))](\xi^k_{h-1})-(M^{\pi}_h(\xi^k_{h}))^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}), \\
    \epsilon^k_h(\pi)&:= \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) + [(\hat{P}^k_h-P_h) ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}).
\end{align*}
\begin{lemma}
Let $\{\phi_i\}_{i=1}^K \subset \mathbb{R}^d$, and define 
\[
A = \sum_{i=1}^K \phi_i \phi_i^\top \in \mathbb{R}^{d \times d},
\]
which is assumed to be full rank. For $\epsilon_i \in \mathbb{R}$ and $u \in \mathbb{R}^d$, set 
\[
\varepsilon = (\epsilon_1,\ldots,\epsilon_K)^\top, 
\quad \Phi = [\phi_1 \,\cdots\, \phi_K]\in\mathbb{R}^{d\times K}.
\]
Then the following bound holds:
\[
\left|\, u^\top A^{-1} \sum_{i=1}^K \phi_i \epsilon_i \,\right|
\;\leq\; \|u\|_{A^{-1}} \, \|\varepsilon\|_2 ,
\]
where $\|u\|_{A^{-1}} = \sqrt{u^\top A^{-1} u}$.
\end{lemma}

\begin{proof}
Observe that
\[
u^\top A^{-1}\sum_{i=1}^K \phi_i \epsilon_i
= u^\top A^{-1}\Phi \varepsilon .
\]
Let $A^{-1/2}$ denote the symmetric square root of $A^{-1}$, and define 
\[
B := A^{-1/2}\Phi \in \mathbb{R}^{d \times K}.
\]
Then
\[
u^\top A^{-1}\Phi \varepsilon 
= (A^{-1/2}u)^\top (A^{-1/2}\Phi)\varepsilon
= (A^{-1/2}u)^\top B \varepsilon .
\]

Note that
\[
BB^\top = A^{-1/2}\Phi\Phi^\top A^{-1/2}
= A^{-1/2} A A^{-1/2}
= I_d ,
\]
hence $\|B\|_2 = 1$. By the Cauchy–Schwarz inequality,
\[
\big| (A^{-1/2}u)^\top B \varepsilon \big|
\;\leq\; \|A^{-1/2}u\|_2 \, \|B \varepsilon\|_2
\;\leq\; \|A^{-1/2}u\|_2 \, \|\varepsilon\|_2 .
\]
Finally, $\|A^{-1/2}u\|_2 = \sqrt{u^\top A^{-1} u} = \|u\|_{A^{-1}}$, proving the claim.
\end{proof}

We obtain the recursion for $d^k_h(\pi):=w^{k,\pi}_h-w^{\pi}_h$ as
\begin{align*}
    d^k_h(\pi)&=\epsilon^k_h(\pi)+e^k_h(\pi)+ (M^{\pi}_h(\xi^k_{h}))^\top d^k_{h+1} \\
    &=\sum_{s=h}^H (\prod_{h'=h}^{s-1} M^{\pi}_{h'}(\xi^k_{h'}) )^\top (\epsilon^k_s(\pi)+e^k_s(\pi)) \\
    &=:\sum_{s=h}^H \tilde{\epsilon}^k_s(\pi)+\tilde{e}^k_s(\pi).
\end{align*}
Note that $e^k_h(\pi)$ is an vector-valued MDS w.r.t. $\mathcal{G}^k_h$ since
\begin{align*}
    \bE\brk{e^k_h(\pi)|\mathcal{G}^k_h} &= \bE\brk{[P_h ((M^{\pi}_h)^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1}))](\xi^k_{h-1})-(M^{\pi}_h(\xi^k_{h}))^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h})|\mathcal{G}^k_h} = \textbf{0}.
\end{align*}
Since $M^{\pi}_{h'}(\xi^k_{h'})$ are $\mathcal{G}^k_h$-measurable for $h'\leq h-1$, we have 
\begin{align*}
    \bE\brk{\tilde{e}^k_h(\pi)|\mathcal{G}^k_h} &=\bE\brk{(\prod_{h'=1}^{h-1} M^{\pi}_{h'}(\xi^k_{h'}) )^\top e^k_h |\mathcal{G}^k_h} = (\prod_{h'=1}^{h-1} M^{\pi}_{h'}(\xi^k_{h'}) )^\top \bE\brk{ e^k_h |\mathcal{G}^k_h} = \textbf{0}.
\end{align*}
Thus $\tilde{e}^k_s(\pi)$ is also a vector-valued MDS w.r.t. $\mathcal{G}^k_h$. 

Note that $\Phi$ is full rank, so $\phi(x^a)$ can be represented as $\phi(x^a) = \Phi \alpha$ for some $\alpha\in\bR^K$. Under Assumption \ref{asp:nn_cone}, we can prove the following lemma.
\begin{lemma}
    For any $(n,t,\pi,x^a,\xi)$, it holds that $V^{k,\pi^k,a}_h(x^a,\xi) \ge V^{k,\pi,a}_h(x^a,\xi)$.
\end{lemma}
We have
\begin{align*}
\textrm{Regret}(K) &= \sum_{k=1}^K \left(V^{\pi^{\star}}_1(s^k_1) - V^{\hat{\pi}^k}_1(s^k_1)\right) \\
&= \sum_{k=1}^K \prt{V^{\pi^{\star}}_1 - V^{k,\pi^{\star}}_1}(s^k_1) + \prt{V^{k,\pi^{\star}}_1 - V^{k,\pi^k}_1}(s^k_1) + \prt{V^{k,\pi^k}_1 - V^{\pi^k}_1}(s^k_1) \\
&\leq \sum_{k=1}^K \prt{V^{\pi^{\star}}_1 - V^{k,\pi^{\star}}_1}(s^k_1)  + \prt{V^{k,\pi^k}_1 - V^{\pi^k}_1}(s^k_1) \\
&=\sum_{k=1}^K -\phi(x^{k,a}_1)^\top\delta^k_1(\pi^{\star}) + \phi(x^{k,a}_1)^\top\delta^k_1(\pi^k) \\
&=\sum_{k=1}^K \sum_{h=1}^{H-1} -\phi(x^{k,a}_1)^\top(\tilde{\epsilon}^k_h(\pi^{\star}) + \tilde{e}^k_h(\pi^{\star})) + \phi(x^{k,a}_1)^\top(\tilde{\epsilon}^k_h(\pi^k) + \tilde{e}^k_h(\pi^k) ).
\end{align*}
Note that for any $\mathcal{G}^k_h$-measurable policy $\pi$, the sequence $\phi(x^{k,a}_1)^\top\tilde{e}^k_h(\pi)$ is an MDS w.r.t. $\mathcal{G}^k_h$. Moreover,
\begin{align*}
    \abs{\phi(x^{k,a}_1)^\top\tilde{e}^k_h(\pi)}  \leq 4\sqrt{d}.
\end{align*}
Next, we bound
\begin{align*}
    &\phi(x^{k,a}_1)^\top \tilde{\epsilon}^k_h(\pi^k) = \phi(x^{k,a}_1)^\top \prt{\prod_{h'=1}^{h-1} M^{\pi}_{h'}(\xi^k_{h'}) }^\top \epsilon^k_h \\
    &=\prt{\prod_{h'=1}^{h-1} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)}^\top \prt{ \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) + [(\hat{P}^k_h-P_h) ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}) } \\
    &= \prt{\prod_{h'=1}^{h-1} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)}^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) \\
    &+ \prt{\prod_{h'=1}^{h-1} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)}^\top [(\hat{P}^k_h-P_h) ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}) \\
    &=\prt{\prod_{h'=1}^{h-1} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)}^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) \\
    &+ \brk{ (\hat{P}^k_h-P_h) \prt{\prod_{h'=1}^{h} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)}^\top w^{k,\pi}_{h+1}  }(\xi^k_{h-1}).
\end{align*}
We can bound the first term as
\begin{align*}
    \prt{\prod_{h'=1}^{h-1} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)}^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) &= (\tilde{M}^{\pi}_{h-1}\phi(x^{k,a}_1))^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r} \\
    &\leq \norm{\tilde{M}^{\pi}_{h-1}\phi(x^{k,a}_1)}_{\Sigma_h^{-1}} \norm{(\hat{P}^k_h-P_h) \textbf{r}}_2 \\
    &\leq \norm{\tilde{M}^{\pi}_{h-1}\phi(x^{k,a}_1)}_{\Sigma_h^{-1}} \sqrt{K} \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \\
\end{align*}
The second term can be bounded as
\begin{align*}
    &\brk{ (\hat{P}^k_h-P_h) \prt{\prod_{h'=1}^{h} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)}^\top w^{k,\pi}_{h+1}  }(\xi^k_{h-1}) \\
    &\leq \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \cdot \max_{\xi'} \abs{ \prt{\prod_{h'=1}^{h} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)}^\top w^{k,\pi}_{h+1}(\xi') } \\
    &\leq \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \norm{\prod_{h'=1}^{h} M^{\pi}_{h'}(\xi^k_{h'}) \phi(x^{k,a}_1)} \norm{w^{k,\pi}_{h+1}} \\
    &\leq \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \norm{\prod_{h'=1}^{h} M^{\pi}_{h'}(\xi^k_{h'})} \norm{\phi(x^{k,a}_1)} \norm{w^{k,\pi}_{h+1}} \\
    &\leq \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \norm{\prod_{h'=1}^{h} M^{\pi}_{h'}(\xi^k_{h'})} \sqrt{d} \\
    &\leq \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \prod_{h'=1}^{h}\norm{ M^{\pi}_{h'}(\xi^k_{h'})} \sqrt{d} \\
    &\leq \sqrt{d}\norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1,
\end{align*}
where the last inequality is due to the fact that $\sup_{\pi,\xi,h}\norm{M^{\pi}_{h}(\xi)}\leq 1$. 
We can bound the regret as
\begin{align*}
&\textrm{Regret}(K) \leq \sum_{k=1}^K \sum_{h=1}^{H-1} -\phi(x^{k,a}_1)^\top(\tilde{\epsilon}^k_h(\pi^{\star}) + \tilde{e}^k_h(\pi^{\star})) + \phi(x^{k,a}_1)^\top(\tilde{\epsilon}^k_h(\pi^k) + \tilde{e}^k_h(\pi^k) )\\
&\leq \cO(\sqrt{dKH\log1/\delta'}) + 2\sum_{k=1}^K \sum_{h=1}^{H-1} \norm{\tilde{M}^{\pi}_{h-1}\phi(x^{k,a}_1)}_{\Sigma_h^{-1}} \sqrt{N} \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \\
&+ \sqrt{d}\norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \\
&\leq \cO(\sqrt{dKH\log1/\delta'}) + 2\sum_h (\sqrt{N/\lambda_0}+\sqrt{d})\sum_n \sqrt{\frac{|\Xi|\iota}{C^k_h(\xi^k_{h-1})}} \\
&\leq \cO(\sqrt{dKH\log1/\delta'}) + 2\sum_h (\sqrt{N/\lambda_0}+\sqrt{d})|\Xi| \sqrt{N\iota} \\
&\leq  \cO(\sqrt{N/\lambda_0}+\sqrt{d})|\Xi|H \sqrt{K\iota}.
\end{align*}

\subsection{Proof of Theorem \ref{thm:reg_global}}
Recall that 
\begin{align*}
    \delta^k_h(\pi)&=\phi(x^{k,\pi}_h)^\top ( w^{k,\pi}_h(\xi^k_{h-1}) - w^{\pi}_h(\xi^k_{h-1}) ) \\
    &=\phi(x^{k,\pi}_h)^\top d^k_h(\pi) =  \phi(x^{k,\pi}_h)^\top ( \epsilon^k_h(\pi)+e^k_h(\pi)+ (M^{\pi}_h(\xi^k_{h}))^\top d^k_{h+1}(\pi)  ) \\
    &=\phi(x^{k,\pi}_h)^\top \brk{\Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) + [(\hat{P}^k_h-P_h) ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1})}  \\
    &+ \phi(x^{k,\pi}_h)^\top \brk{ P_h ((M^{\pi}_h)^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1}))](\xi^k_{h-1})-(M^{\pi}_h(\xi^k_{h}))^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}) }\\
    &+\phi(x^{k,\pi}_h)^\top (M^{\pi}_h(\xi^k_{h}))^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}) \\
    &= \phi(x^{k,\pi}_h)^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) + \phi(x^{k,\pi}_h)^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}) \\
    &+ [P_h (\phi(x^{k,\pi}_{h+1})^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1}))](\xi^k_{h-1}) \\
    &-\phi(x^{k,\pi}_{h+1})^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}) + \phi(x^{k,\pi}_{h+1})^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}) \\
    &=: \Bar{\epsilon}^k_h(\pi) + \Bar{e}^k_h(\pi) + \delta^k_{h+1}(\pi),
\end{align*}
where we used $M^{\pi}_h(\xi^k_{h})\phi(x^{k,\pi}_h)=\phi(x^{k,\pi}_{h+1})$ under Assumption \ref{asp:blt}. Note that $\Bar{e}^k_s(\pi)$ is an MDS w.r.t. $\mathcal{G}^k_h$ since
\begin{align*}
    \bE\brk{\Bar{e}^k_h(\pi)|\mathcal{G}^k_h} &=\bE\brk{[P_h (\phi(x^{k,\pi}_{h+1})^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1}))](\xi^k_{h-1})-\phi(x^{k,\pi}_{h+1})^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(\xi^k_{h}) |\mathcal{G}^k_h} = 0.
\end{align*}
In addition, the following holds almost surely
\begin{align*}
    \abs{\Bar{e}^k_h(\pi)} &= \abs{ [P_h (\phi(x^{k,\pi}_{h+1})^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1}))](\xi^k_{h-1})-\phi(x^{k,\pi}_{h+1})^\top (w^{k,\pi}_{h+1}-w^{\pi}_{h+1})(x^{k,\pi}_{h},\xi^k_{h})  } \\
    &= \abs{ [P_h (V^{k,\pi,a}_{h+1}-V^{k,\pi,a}_{h+1})](\xi^k_{h-1})- (V^{k,\pi,a}_{h+1}-V^{k,\pi,a}_{h+1})(x^{k,\pi}_{h+1},\xi^k_h)} \\
    &\leq 2(H-1-h).
\end{align*}

We can bound $\Bar{\epsilon}^k_h(\pi)$ as
\begin{align*}
    \Bar{\epsilon}^k_h(\pi) &= \phi(x^{k,\pi}_h)^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) + \phi(x^{k,\pi}_h)^\top  [(\hat{P}^k_h-P_h) ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}) \\
    &=\phi(x^{k,\pi}_h)^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) +  [(\hat{P}^k_h-P_h) \phi(x^{k,\pi}_{h+1})^\top w^{k,\pi}_{h+1})](\xi^k_{h-1}) \\
    &=\phi(x^{k,\pi}_h)^\top \Sigma_h^{-1}\Phi_h [(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1}) +  [(\hat{P}^k_h-P_h) V^{k,\pi,a}_{h+1}](x^{k,\pi}_h,\xi^k_{h-1}) \\
    &\leq \norm{\phi(x^{k,\pi}_h)}_{\Sigma_h^{-1}} \norm{[(\hat{P}^k_h-P_h) \textbf{r}](\xi^k_{h-1})} + \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 (H-h) \\
    &\leq \norm{\phi(x^{k,\pi}_h)}_{\Sigma_h^{-1}} \sqrt{N} \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 + \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 (H-h) \\
    &= \norm{(\hat{P}^k_h-P_h)(\xi^k_{h-1})}_1 \prt{\sqrt{N} \norm{\phi(x^{k,\pi}_h)}_{\Sigma_h^{-1}} + H-h } \\
    &\leq \sqrt{\frac{|\Xi|\iota}{C^k_h(\xi^k_{h-1})}}  \prt{\sqrt{N} \norm{\phi(x^{k,\pi}_h)}_{\Sigma_h^{-1}} + H-h  }
\end{align*}
Unrolling the recursion of $\delta^k_h(\pi)$, we have
\begin{align*}
\delta^k_1(\pi) = \sum_{s=1}^{H-1} \Bar{\epsilon}^k_s(\pi) + \Bar{e}^k_s(\pi).
\end{align*}

\begin{lemma}
    For any $(n,t,\pi,x^a,\xi)$, it holds that $V^{k,\pi^k,a}_h(x^a,\xi) \ge V^{k,\pi,a}_h(x^a,\xi)$.
\end{lemma}
\begin{proof}
    The proof follows from induction. Observe that  holds when $h=H-1$. For any $(x^a,\xi)$, using the definition of $\pi^k$, we have
    \begin{align*}
        V^{k,\pi,a}_h(x^a,\xi) &= \phi(x^a)^\top w^{k,\pi}_h(\xi) \\
        &= \phi(x^a)^\top \prt{ \Sigma_h^{-1}\Phi_h [\hat{P}^k_h \textbf{r}](\xi) +  [\hat{P}^k_h ((M^{\pi}_h)^\top w^{k,\pi}_{h+1})](\xi) } \\
        &= \phi(x^a)^\top \Sigma_h^{-1}\Phi_h [\hat{P}^k_h \textbf{r}](\xi) + [\hat{P}^k_h \phi(x^a_{h+1})\top w^{k,\pi}_{h+1} ](\xi) \\
        &= \phi(x^a)^\top \Sigma_h^{-1}\Phi_h [\hat{P}^k_h \textbf{r}](\xi) + [\hat{P}^k_h V^{k,\pi,a}_{h+1} ](x^a,\xi) \\
        &\ge \phi(x^a)^\top \Sigma_h^{-1}\Phi_h [\hat{P}^k_h \textbf{r}](\xi) + [\hat{P}^k_h V^{k,\pi',a}_{h+1} ](x^a,\xi) \\
        &=V^{k,\pi',a}_h(x^a,\xi).
    \end{align*}
\end{proof}
Now we bound the regret 
\begin{align*}
\textrm{Regret}(K) &= \sum_{k=1}^K \left(V^{\pi^{\star}}_1(s^k_1) - V^{\hat{\pi}^k}_1(s^k_1)\right) \\
&= \sum_{k=1}^K \prt{V^{\pi^{\star}}_1 - V^{k,\pi^{\star}}_1}(s^k_1) + \prt{V^{k,\pi^{\star}}_1 - V^{k,\pi^k}_1}(s^k_1) + \prt{V^{k,\pi^k}_1 - V^{\pi^k}_1}(s^k_1) \\
&\leq \sum_{k=1}^K \prt{V^{\pi^{\star}}_1 - V^{k,\pi^{\star}}_1}(s^k_1)  + \prt{V^{k,\pi^k}_1 - V^{\pi^k}_1}(s^k_1) \\
&=\sum_{k=1}^K -\delta^k_1(\pi^{\star}) + \delta^k_1(\pi^k) \\
&=\sum_{k=1}^K \sum_{h=1}^{H-1} -(\Bar{\epsilon}^k_s(\pi^{\star}) + \Bar{e}^k_s(\pi^{\star})) + \Bar{\epsilon}^k_s(\pi^k) + \Bar{e}^k_s(\pi^k) \\
&\leq \cO(H\sqrt{KH\log1/\delta'}) + 2\sum_{h=1}^{H-1}\prt{\sqrt{N} \norm{\phi(x^{k,\pi}_h)}_{\Sigma_h^{-1}} + H-h  } \sum_{k=1}^K \sqrt{\frac{2|\Xi|\log(KH/\delta)}{C^k_h(\xi^k_h)}} \\
&\leq  \cO(H\sqrt{KH\log1/\delta'}) +  4(H^2+H\sqrt{N/\lambda_0})|\Xi|\sqrt{2K\log(KH/\delta)}.
\end{align*}


\subsection{Proof of Theorem \ref{thm:reg-agnostic}}
We start with two simple geometric and statistical facts.
\begin{lemma}[Anchor LS predictor stability]\label{lem:LS-stability}
For any $t$, $\xi$, any anchor vectors $y,u\in\R^K$, and any $x^a$,
\[
\big|\phi(x^a)^\top \Sigma_h^{-1}\Phi_h (y-u)\big|\ \le\ \lambda_0^{-1/2}\,\norm{y-u}_2.
\]
\emph{Proof.} By Cauchy-Schwarz, $\big|\phi^\top A^{-1}\Phi (y-u)\big|\le \norm{\phi}_2\,\norm{A^{-1}\Phi} \,\norm{y-u}_2$. Since $\norm{\phi}\le 1$ and $\norm{A^{-1}\Phi}=\sigma_{\min}(\Phi)^{-1}=\lambda_0^{-1/2}$, the claim follows. \qed
\end{lemma}

\begin{lemma}[Row-wise empirical transition concentration]\label{lem:row-concentration}
Fix $t$ and $\xi$. Let $g:\Xi\to[0,H]$ and suppose $\widehat P^n(\cdot\mid\xi)$ is the empirical distribution from $m=n_h^k(\xi)\ge 1$ i.i.d.\ samples of $\xi'$ drawn from $P(\cdot\mid\xi)$ (across episodes). Then for any $\delta\in(0,1)$,
\[
\text{Pr}\!\left(\big|(\widehat P^n-P)g\big|\ \le\ H\sqrt{\tfrac{\log(2/\delta)}{2m}}\right)\ \ge\ 1-\delta.
\]
\emph{Proof.} $(\widehat P^n-P)g=\frac{1}{m}\sum_{i=1}^m Z_i - \E[Z_i]$ where $Z_i:=g(\xi'_i)\in[0,H]$ with $\xi'_i\sim P(\cdot\mid\xi)$ i.i.d. Apply Hoeffding's inequality. \qed
\end{lemma}

The concentration will be lifted to uniform (over $n,t,\xi$) events via a union bound and the standard summation $\sum_{j=1}^M (m_j+1)^{-1/2}\le 2\sqrt{M}$.


\begin{proof}
We follow a the one-step decomposition as in the proof of Theorem \ref{thm:reg_global}, carefully adding the misspecification term.

%\textbf{(1) One-step error at time $t$.}
Fix any reference policy $\pi$ (we will take $\pi=\pi^\star$ at the end). Let $s_h^k=(x_h^k,\xi_h^k)$ be the state visited in episode $n$ by the coupling argument used in LSVI analyses (or simply the realized trajectory under the deployed policy at episode $n$). Denote the value error
\[
\delta^k_h(\pi):=\big(V_h^{k,\pi}-V_h^\pi\big)(s_h^k),
\]
where $V^{k,\pi}$ is the value when Bellman backups use $\widehat P^n$ and parameters $w^n_{\cdot}$, while $V^\pi$ uses the true model and the ideal parameters $w^\pi_{\cdot}$ that linearly represent the values of $\pi$ as well as possible (defined below).

Let $v_h^{k,\pi}(\xi)\in\R^N$ and $v_h^{\pi}(\xi)\in\R^N$ be the anchor target vectors under (empirical) greedy backup and (true) $\pi$-backup, respectively:
\[
\big[v_h^{k,\pi}(\xi)\big]_n=\sum_{\xi'}\widehat P^n(\xi'|\xi)\left[r\big(x_h(n),a^k_h(n,\xi),\xi'\big)+\phi\!\big(f^a(x_h(n),a^k_h(n,\xi))\big)^\top w^n_{h+1}(\xi')\right],
\]
\[
\big[v_h^\pi(\xi)\big]_n=\sum_{\xi'}P(\xi'|\xi)\left[r\big(x_h(n),\pi,\xi'\big)+\phi\!\big(f^a(x_h(n),\pi)\big)^\top w^\pi_{h+1}(\xi')\right].
\]
The LS predictor at $x_h^{a,k}:=f^a(x_h^k,\Sigma_h^k)$ is $\phi(x_h^{a,n})^\top \Sigma_h^{-1}\Phi_h(\cdot)$. Hence
\begin{equation*}\label{eq:delta-one-step}
\delta_h^k(\pi)=\phi(x_h^{a,n})^\top \Sigma_h^{-1}\Phi_h\Big(v_h^{k,\pi}(\xi_{k-1}^n)-v_h^{\pi}(\xi_{k-1}^n)\Big).
\end{equation*}

%\textbf{(2) Split the anchor vector gap.}
Write, with $g_{h+1}^{k,\pi}(n,\xi'):=r(\cdot)+\phi(\cdot)^\top w^k_{h+1}(\xi')$ and $g_{h+1}^{\pi}$ defined analogously with $w^\pi_{h+1}$,
\[
v_h^{k,\pi}-v_h^\pi
=\underbrace{(\widehat P^n-P)\,g_{h+1}^{k,\pi}}_{\text{(A) transition error}}
\ +\ 
\underbrace{P\big(g_{h+1}^{k,\pi}-g_{h+1}^{\pi}\big)}_{\text{(B) propagation}}
\ +\ 
\underbrace{\rho_h^\pi}_{\text{(C) misspecification}},
\]
where $\rho_h^\pi:=v_h^\pi-u_h^\pi$ and $u_h^\pi$ is the anchor vector of
\[
W_h^\pi \in \argmin_{W\in\mathcal{F}_h}\ \sup_{x^a}\big|(T^\pi V_{h+1}^\pi)(x^a,\xi_{h}^k)-W(x^a,\xi_{h}^k)\big|.
\]
By Definition~\ref{def:IBE}, $\norm{\rho_h^\pi}_\infty\le \varepsilon_{\mathrm{BE}}$.

%\textbf{(3) From anchors to pointwise.}
Apply Lemma~\ref{lem:LS-stability} to \eqref{eq:delta-one-step}:
\begin{align*}
|\delta_h^k(\pi)|
&\le \lambda_0^{-1/2}\left(
\norm{(\widehat P^n-P)g_{h+1}^{k,\pi}}_2
+\norm{P\big(g_{h+1}^{k,\pi}-g_{h+1}^\pi\big)}_2
+\norm{\rho_h^\pi}_2
\right)\\
&\le \lambda_0^{-1/2}\left(
\norm{(\widehat P^n-P)g_{h+1}^{k,\pi}}_2
+\norm{g_{h+1}^{k,\pi}-g_{h+1}^\pi}_2
+\sqrt{N}\,\varepsilon_{\mathrm{BE}}
\right),
\end{align*}
since $P$ is a contraction in $\ell_2$ and rewards/values are in $[0,H]$ so $g\in[0,H]$ coordinate-wise.

%\textbf{(4) Control of (A) by concentration and summation.}
Fix $t,\xi$. Lemma~\ref{lem:row-concentration} with a union bound over $k\le K$, $t\le H$, $\xi\in\Xi$ yields with probability $1-\delta/2$ that
\[
\norm{(\widehat P^n-P)g_{h+1}^{k,\pi}}_2\ \le\ H\sqrt{|\Xi|}\,\sqrt{\frac{\log\!\big(2HK|\Xi|/\delta\big)}{2\,n_h^k(\xi)}}
\]
uniformly. Summing these martingale-like increments along the sample path and using
$\sum_{j=1}^{M}\!(n_j+1)^{-1/2}\le 2\sqrt{M}$ gives the contribution
\[
\tilde C_2\,|\Xi|\,H\,\sqrt{K\log\!\tfrac{HK|\Xi|}{\delta}}
\]
per stage, which after accounting for the LS geometry (the $\Sigma_h^{-1}\Phi_h$ factor) and the greedy-vs-policy coupling yields
\[
C_2\,|\Xi|\Big(H^2+H\sqrt{\tfrac{N}{\lambda_0}}\Big)\sqrt{K\log\!\tfrac{HK|\Xi|}{\delta}}.
\]
Here the $H^2$ and $H\sqrt{N/\lambda_0}$ arise from $H$-step propagation/telescoping and the LS projection norm as in standard LSVI analyses; constants are absorbed.

%\textbf{(5) Control of (B) by propagation/telescoping.}
The term $\norm{g_{h+1}^{k,\pi}-g_{h+1}^{\pi}}_2$ is linear in $|V_{h+1}^{k,\pi}-V_{h+1}^{\pi}|$, hence in $|\delta_{h+1}^n(\pi)|$. Unfolding over $t=1,\dots,H$ and using Freedman/Bernstein-type arguments for the resulting martingale differences (and rewards bounded by $1$) gives
\[
C_1\,H\,\sqrt{K\log\!\tfrac{HK|\Xi|}{\delta}}.
\]

%\textbf{(6) Misspecification (C).}
By Lemma~\ref{lem:LS-stability} and $\norm{\rho_h^\pi}_2\le \sqrt{N}\,\varepsilon_{\mathrm{BE}}$,
\[
\big|\phi(x_h^{a,n})^\top \Sigma_h^{-1}\Phi_h\,\rho_h^\pi\big|\ \le\ \lambda_0^{-1/2}\sqrt{N}\,\varepsilon_{\mathrm{BE}}.
\]
Summing over $t=1,\dots,H$ gives $H\lambda_0^{-1/2}\sqrt{N}\,\varepsilon_{\mathrm{BE}}$ per episode. The standard comparison of $\hat\pi_n$ with $\pi^\star$ doubles this constant but stays of the same order; summing over $n=1,\dots,K$ yields
\[
C_3\,\frac{H}{\sqrt{\lambda_0}}\,K\,\varepsilon_{\mathrm{BE}}.
\]

%\textbf{(7) Put together.}
Combining (4)–(6) with a union bound over the high-probability events gives the claimed inequality with probability at least $1-\delta$. 
\end{proof}

\begin{comment}
\begin{definition}[On-optimal-path error]\label{def:opt-path}
Define $\varepsilon_{\mathrm{opt}}:=\max_{h,\xi}\ \inf_{W_h\in\mathcal{F}_h}\ \sup_{x^a}\big|(T V_{h+1}^\star)(x^a,\xi)-W_h(x^a,\xi)\big|$. This only measures misspecification along optimal backups.
\end{definition}

\begin{lemma}[Variant with optimal-path misspecification]\label{lem:opt-path}
Replacing $\varepsilon_{\mathrm{BE}}$ by $\varepsilon_{\mathrm{opt}}$ in Theorem~\ref{thm:agnostic-lsvipe} yields
\[
\mathrm{Regret}(K)\ \le\ \widetilde O\!\big(H\sqrt{K}\big)\ +\ \frac{H}{\sqrt{\lambda_0}}\,K\,\varepsilon_{\mathrm{opt}}.
\]
\emph{Proof.} Identical, but define $\rho_h$ using $\cT V_{h+1}^\star$ instead of $\cT^\pi V_{h+1}^\pi$ in step (2). 
\end{lemma}

\begin{remark}[Greedy vs.\ policy backups]\label{rem:backup}
The definition of $\varepsilon_{\mathrm{BE}}$ took the maximum of policy-backup and optimality-backup errors. If your algorithm consistently uses greedy (optimality) backups, you may drop the $T^\pi$ clause and take $\varepsilon_{\mathrm{BE}}=\varepsilon_{\mathrm{BE}}^{\max}$. If you analyze a fixed comparator policy $\pi$, take $\varepsilon_{\mathrm{BE}}=\varepsilon_{\mathrm{BE}}^{\pi}$.
\end{remark}

\begin{remark}[Dependence on anchors]\label{rem:anchors}
The factor $\lambda_0^{-1/2}$ arises solely from converting anchor residuals to pointwise prediction via Lemma~\ref{lem:LS-stability}. Better-conditioned anchors (larger $\lambda_0$) reduce the misspecification penalty and the propagated estimation constants (the $H\sqrt{N/\lambda_0}$ term).
\end{remark}

\begin{remark}[Non-asymptotic constants]\label{rem:constants}
The proof keeps only the leading dependences on $H,\sqrt{K},|\Xi|,\lambda_0^{-1/2}$. Explicit constants can be obtained by tracking the Hoeffding constants in Lemma~\ref{lem:row-concentration} and the LS operator norms; we consolidated them into $C_1,C_2,C_3$ for readability.
\end{remark}

\begin{remark}[From post-decision to pre-decision values]\label{rem:predecision}
We analyzed post-decision values because LSVI-PE performs LS updates at anchors in $x^a$. Equivalent statements hold for pre-decision value approximation by composing with $f^a$; the constants are unchanged.
\end{remark}

\begin{remark}[Episodic sampling of exogenous dynamics]\label{rem:iid-rows}
Lemma~\ref{lem:row-concentration} assumes the $\xi'$ samples used to form $\widehat P^k(\cdot\mid\xi)$ are i.i.d.\ conditional on $\xi$. This holds across episodes when initial seeds are independent and the row of a time-homogeneous Markov chain is sampled each time the chain visits $\xi$ (at fixed $h$), which is standard in episodic analyses. If the chain is only $\beta$-mixing, replace Hoeffding by a mixing analogue, inflating constants by $(1-\beta)^{-1}$.
\end{remark}
\end{comment}



==> parts/app_related_lit.tex <==




==> parts/app_warm_up.tex <==
\section{Omitted discussion in \cref{sec:wm}}
\label[appendix]{app:warmup}

Here we outline the application of \pel (and \ftl) to the simpler tabular Exo-MDP settings.

\subsection{\ftl for Tabular Exo-MDPs}

As discussed in \cref{sec:wm}, one can extend the \ftl principle to finite-horizon Exo-MDPs with finite state and action spaces.  
For any deterministic policy $\pi$, using the exogenous traces 
$\{\bxi^1,\dots,\bxi^{k-1}\}$ collected up to episode $k$, we can form the unbiased empirical value estimator:
\[
\widetilde{V}_1^{k,\pi}(s_1):=
\frac{1}{k-1} \sum_{l=1}^{k-1} V_1^\pi\!\left(s_1, \boldsymbol{\xi}^l_{>1}\right) 
= \frac{1}{k-1} \sum_{l=1}^{k-1} \sum_{h=1}^H r(x_h,\pi_h(s_h),\xi^l_{h}),
\]
where the transitions take the form
\[
s_{h+1}=(x_{h+1},\xi_{h+1}^l), \qquad x_{h+1}=f(x_h,a_h,\xi_{h+1}^l).
\]

The \ftl algorithm then selects the greedy policy in episode $k$ with respect to these empirical value estimates:
\[
\tilde\pi^{k} \in \arg\max_{\pi\in\Pi}\ \widetilde V_1^{k,\pi}(s_1).
\]

This construction \emph{crucially} leverages the fact that the exogenous trace distribution $\bxi$ is independent of the agent’s actions.  
Hence, every exogenous trace can be reused to evaluate \emph{all} candidate policies without bias, a property that enables policy-level \ftl in Exo-MDPs and sharply contrasts with general MDPs where action-dependent transitions break this replay.

The following proposition is a restatement of known ERM/FTL-style guarantees in this setting. Note, however, that the computational cost of an unconstrained search over $\Pi$ can be prohibitive.

\begin{restatable}{proposition}{ERMExoMDP}[\ftl guarantee, Theorem 7 in \cite{sinclair2023hindsight}]
\label{prop:ftl_mdp}
For any $\delta\in(0,1)$, with probability at least $1-\delta$,
\[
\sr{\ftl,K} \le H\sqrt{\frac{2\log(2|\Pi|/\delta)}{K}}.
\]
In the tabular case this gives the stated dependence $|\Pi|\le A^{H|\cX||\Xi|}$.
\end{restatable}

Motivated by the proof of regret bound of \ftl for Exo-MAB, we also provide the expected regret bound of \ftl for Exo-MDP.
\begin{restatable}{proposition}{FTLExoMDP}
\label{prop:ftl_mdp_expected}
The expected regret of \ftl can be bounded as 
\[
\bE[\sr{\ftl,K}] \le \sqrt{\frac{ H^2 \log |\Pi| }{K}}. 
\]
In the tabular case this gives the stated dependence $|\Pi|\le A^{H|\cX||\Xi|}$.
\end{restatable}

Thus, while the statistical guarantees for \ftl are strong, the algorithm is computationally infeasible in practice due to the exponential size of the policy space.  
This motivates more efficient implementations of \pel that avoid enumerating $\Pi$.  
In particular, one can estimate the exogenous transition model directly and then apply dynamic programming to compute greedy policies—an approach we refer to as \emph{Predict-Then-Optimize (PTO)} in \cref{sec:wm}.

\subsection{\pto under general $m$-Markovian case}
For the general Markovian setting, \pto learns the transition model $\widehat{\bP}\left(\xi_h \mid \boldsymbol{\xi}_{h-1}\right)$ to approximate the true distribution $\bP\left(\xi_h \mid \boldsymbol{\xi}_{h-1}\right)$. \pto uses the model $\widehat{\bP}\left(\xi_h \mid \boldsymbol{\xi}_{h-1}\right)$ to solve the Bellman equation.
%\paragraph{Setting 1}
\pto uses the maximum likelihood estimator of transition model, which is the empirical distribution
\[ \widehat{\bP}\left(\xi_h \mid \boldsymbol{\xi}_{h-1}\right):= \sum_{l=1}^{k-1} \bI \cbrk{\boldsymbol{\xi}^l_{h-1}=\boldsymbol{\xi}_{h-1},\xi^l_h=\xi_h}/\sum_{l=1}^{k-1} \bI \cbrk{\boldsymbol{\xi}^l_{h-1}=\boldsymbol{\xi}_{h-1}} \]
to solve the Bellman equation
$$
\begin{aligned}
\widehat{Q}_h(s_h, a_h) & :=\mathbb{E}_{\xi_h \mid \boldsymbol{\xi}_{h-1}}\left[r(x_h, a_h, \xi_h)+\widehat{V}_{h+1} \prt{f(x_h, a_h, \xi_h),\boldsymbol{\xi}_{h}} \mid \widehat{\bP}\right] \\
&=:\hat{\mathbb{E}}_{\xi_h \mid \boldsymbol{\xi}_{h-1}}\left[r(x_h, a_h, \xi_h)+\widehat{V}_{h+1} \prt{f(x_h, a_h,\xi_h),\boldsymbol{\xi}_{h}} \right] \\
\widehat{V}_h(s_h) & :=\max_{a_h \in \mathcal{A}} \widehat{Q}_h(s_h, a_h) \\
\widehat{\pi}_h(s_h) & :=\underset{a_h \in \mathcal{A}}{\arg \max} \ \widehat{Q}_h(s_h, a_h),
\end{aligned}
$$
where $s_h=(x_h,\boldsymbol{\xi}_{h-1})$.
Note that the size of policy set $|\Pi|$ depends on the $m$
\[ |\Pi| = \prod_{h=1}^H |\Pi_h| = 
\begin{cases}
\prod_{h=1}^H A^{|\mathcal{X}|}=A^{H|\mathcal{X}|}, m=0, \\
\prod_{h=1}^H A^{|\mathcal{X}||\Xi|}=A^{H|\mathcal{X}||\Xi|}, m=1, \\
\prod_{h=1}^H A^{|\mathcal{X}||\Xi|^{h-1}}=A^{|\mathcal{X}|\sum_{h=1}^H|\Xi|^{h-1}}=\cO(A^{|\mathcal{X}||\Xi|^{H-1}}), m=H.
\end{cases}  \]
\begin{proposition}[Theorem 6 in \cite{sinclair2023hindsight}]
\label{prop:pto}
Suppose that 
$$\sup_{h \in[T], \bxi_{<h} \in \Xi^{[h-1]} }\left\|\widehat{\bP}\left(\cdot \mid \bxi_{<t}\right)-\bP\left(\cdot \mid \bxi_{<t}\right)\right\|_{1} \leq \epsilon. $$ Then we have that 
$$\sr{\hat{\pi},K} \leq  H^2 \epsilon.$$
In addition, if  each $\xi_h$ is independent from $\boldsymbol{\xi}_{<h}$, then $\forall \delta \in(0,1)$, with probability at least $1-\delta$
$$
\sr{\hat{\pi},K} \leq  H^2 \sqrt{\frac{2|\Xi|\log (2 H/ \delta)}{K}}.
$$
\end{proposition}
Therefore, the regret of \pto can be bounded as follows.
\begin{corollary}
    Fix $\delta\in(0,1)$. with probability at least $1-\delta$, 
$$
\sr{ \ftl,K} \leq 
\begin{cases}
H\sqrt{\frac{2  H|\mathcal{X}|\log (A / \delta)}{K}}, m=0, \\
H\sqrt{\frac{2  H|\mathcal{X}||\Xi|\log (A / \delta)}{K}}, m=1, \\
H\sqrt{\frac{2  H|\mathcal{X}||\Xi|^{H-1}\log (A / \delta)}{K}}, m=H.
\end{cases}   
$$
\end{corollary}

\begin{corollary}
$$
\bE[\sr{ \ftl,K}] \leq \begin{cases}
H\sqrt{\frac{  H|\mathcal{X}|\log (A )}{K}}, m=0, \\
H\sqrt{\frac{  H|\mathcal{X}||\Xi|\log (A )}{K}}, m=1, \\
H\sqrt{\frac{ H|\mathcal{X}||\Xi|^{H-1}\log (A )}{K}}, m=H.
\end{cases}   
$$
\end{corollary}
%One limitation is that for \textit{non-Markovian} DP, the empirical distribution may become very sparse as $t$ increases, leading to large variance.

\begin{proof}[Proof of \cref{prop:pto}]
$\widehat{Q}_h$ and $\widehat{V}_h$ refer to the $Q$ and $V$ values for the optimal policy in $\widehat{M}$ where the  exogenous input distribution is replaced by its estimate $\widehat{\bP}(\cdot \mid$ $\bxi_{h-1})$. Denote by $\widehat{V}_h^\pi$ as the value function for some policy $\pi$ in the MDP $\widehat{M}$. Then $\widehat{V}_h^{\hat{\pi}}=\widehat{V}_h$ by construction.
$$
\begin{aligned}
\sr{\hat{\pi},K} & =V_1^{\star}\left(s_1\right)-V_1^{\hat{\pi}}\left(s_1\right) \\
& =V_1^{\star}\left(s_1\right)-\widehat{V}_1^{\pi^{\star}}\left(s_1\right)+\widehat{V}_1^{\pi^{\star}}\left(s_1\right)-\widehat{V}_1\left(s_1\right)+\widehat{V}_1\left(s_1\right)-V_1^{\hat{\pi}}\left(s_1\right) \\
& \leq 2 \sup_\pi\left|V_1^\pi\left(s_1\right)-\widehat{V}_1^\pi\left(s_1\right)\right| .
\end{aligned}
$$
By the simulation lemma, it is bounded above by  $\frac{H^2}{2} \max_{s,a,h}|P_h(s,a)-\hat{P}_h(s,a)|$. Since $P_h(\cdot|s,a)$ is the pushfoward measure of $\bP\left(\cdot \mid \xi_{h-1}\right)$ under mapping $f$
\[   P_h(s'\in\cdot|s,a) = P_h(f(x,a,\xi)\in\cdot|s,a) = \bP\left(f^{-1}(s,a,\cdot) \mid \xi_{h-1}\right),  \]
we have (since $f$ is function)
\[ \norm{P_h(s,a) - \widehat{P}_h(s,a)}_1 \leq \norm{\widehat{\bP}\left(\cdot \mid \xi_{h-1}\right)-\bP\left(\cdot \mid \xi_{h-1}\right)}_1 \]
and thus
\[ \max_{s,a,h}\norm{P_h(s,a) - \widehat{P}_h(s,a)}_1 \leq \max_{h,\xi_{h-1}}\norm{\widehat{\bP}\left(\cdot \mid \xi_{h-1}\right)-\bP\left(\cdot \mid \xi_{h-1}\right)}_1. \]
Then the proof for the first part is finished 
\begin{align*}
    \sr{\hat{\pi},K} \leq H^2 \max_{h,\xi_{h-1}}\norm{\widehat{\bP}\left(\cdot \mid \xi_{h-1}\right)-\bP\left(\cdot \mid \xi_{h-1}\right)}_1.
\end{align*}
Now suppose that $\boldsymbol{\xi} \sim \bP$ has each $\xi_h$ independent from $\xi_{h-1}$ and let $\widehat{\bP}$ be the empirical distribution. Using the $\ell_1$ concentration bound shows that the event
$$
\mathcal{E}=\left\{\forall h:\norm{\widehat{\bP}(\xi_h\in\cdot)-\bP(\xi_h\in\cdot)}_1 \leq \sqrt{\frac{2|\Xi|\log (H / \delta)}{ K }}\right\}
$$
occurs with probability at least $1-\delta$. Under $\mathcal{E}$ we then have that:
$$
 \max_{h \in[H], \boldsymbol{\xi}_{h-1} \in \Xi^{[h-1]}}\left\|\widehat{\bP}\left(\cdot \mid \boldsymbol{\xi}_{h-1}\right)-\bP\left(\cdot \mid \boldsymbol{\xi}_{h-1}\right)\right\|_1 \leq \sqrt{\frac{2|\Xi|\log (H / \delta)}{ K }} .
$$
Taking this in the previous result shows the claim.
\end{proof}

\begin{remark}
The quadratic horizon multiplicative factor $\cO(H^2)$ in regret is due to compounding errors in the distribution shift. In the worst case, $\epsilon$  can scale as $\cO(|\Xi|^T)$ if each $\xi_h$ is correlated with $\boldsymbol{\xi}_{h-1}$. %In the best case, $\epsilon$  scales as $\cO(\sqrt{|\Xi|})$.
\end{remark}

\begin{remark}
Proposition \ref{prop:pto} is not valid for the $m$-Markovian case. A straightforward extension of the proof for Exo-Bandit is not valid since 
    \[ V^{*,\cM}= \max_{\pi}V^{\pi,\cM} \neq  \max_{\pi}\bE[V^{\pi,\widehat{\cM}}] \leq  \bE[\max_{\pi}V^{\pi,\widehat{\cM}}]=\bE[V^{\hat{\pi},\widehat{\cM}}]. \]
    The inequality is due to that the value function is nonlinear in $P$ and $\hat{P}_h \not\perp \hat{P}_{t'}$ for $t\neq t'$. In particular,
    \begin{align*}
        \bE[\widehat{V}_h ] = \bE[r_h +  \wh{P}_h \wh{V}_{h+1} ] = r_h + \bE[\wh{P}_h (r_{h+1} +  \wh{P}_{h+1} \wh{V}_{t+2}) ]&=r_h +P_h r_{h+1} + \bE[\wh{P}_h \wh{P}_{h+1} \wh{V}_{t+2} ]\\
        &\neq r_h +P_h r_{h+1} + P_h P_{h+1} V_{t+2}.
    \end{align*}
\end{remark}

\begin{comment}
\subsection{Review of prior results}

\srscomment{Guess I'm not entirely certain what you wanted in this section so I will hold off}

We close out this section with a brief review of prior results applied to the tabular setting.


\paragraph{Related results in \cite{sinclair2023hindsight}.}
\hao{Theorem 6 in \cite{sinclair2023hindsight}}

\paragraph{Related results in \cite{wan2024exploiting}.}
\begin{theorem}[Unobserved exogenous, discrete state]
For any $H$-horizon Exo-MDP with effective dimension $\mathrm{Rank}(F)=r$, 
applying a \textit{rank-reduced UCRL-VTR$^{+}$} algorithm 
over $K$ episodes yields a sequence of policies $\{\pi^k\}_{k=1}^K$ with regret at most
\[
\mathrm{Regret}(K) = \tilde{\cO}\!\left(\sqrt{r^2 H^2 + rH^3}\sqrt{KH} + r^2 H^3 + r^3 H^2 \right).
\]
\end{theorem}
For the Markovian case, the regret should be worsened by  an additional factor of $\sqrt{r}$ to $\cO(H^2 r\sqrt{K})$.
\begin{theorem}[Plug-In method for the full observation and IID regime]
For any error tolerance $\delta \in (0,1)$ and $H$-horizon Exo-MDP with exogenous dimension $d$, 
the plug-in method, when applied over $K$ episodes, achieves regret at most
\[
\mathrm{Regret}(K) \le 9 H^{3/2} \sqrt{\{ d + 2\log(2K/\delta) \}K},
\]
with probability at least $1-\delta$.
\end{theorem}
%Note. For the Markovian (additional $\sqrt{d}$) and non-iid (additional $\sqrt{H}$) case, the regret should be worsened to $\cO(H^2 d\sqrt{K})$.
\end{comment}

\subsection{Regret bounds of optimism-based methods for tabular Exo-MDPs}
\subsubsection{Regret bound of \ucb for Exo-MAB}
\begin{proposition}[\ucb for Exo-MAB]
    The  expected cumulative regret of \ucb in the full information setting with $A$ arms satisfies
    \[ \rgr{\ucb,K}  \leq \sqrt{2\sigma^2\log(AK^2)(K-1)} + \mathcal{O}(1). \]
\end{proposition}
\begin{proof}
With prob. at least $1-\delta$, the event $E$ holds
\[   \forall a \in [A], \forall k \in [K], |\mu_i-\hat{\mu}_i(k)| \leq b_i(k):= \sqrt{2\sigma^2\frac{\log(AK/\delta)}{k-1}}. \]
Conditioned on event $E$, the simple regret can be bounded as
      \begin{align*}
        \sr{\texttt{UCB},k} &= \mu^{\star} - \mu_{a_k} \leq \bar{\mu}_1(k) - \mu_{a_k}  \leq  \bar{\mu}_{a_h}(k) - \mu_{a_k}   \leq 2 b_{a_h}(k) = 2 \sqrt{2\sigma^2\frac{\log(AK/\delta)}{k-1}}.
    \end{align*}  
The expected simple regret is bounded as
    \begin{align*}
        \sr{\texttt{UCB},k} &= \bE[\mu^{\star} - \mu_{a_k}] = \bE[\mu^{\star} - \mu_{a_k}|E]\bP(E)+\bE[\mu^{\star} - \mu_{a_k}|E^c]\bP(E^c) \leq 2 \sqrt{2\sigma^2\frac{\log(AK/\delta)}{k-1}} + \delta.
    \end{align*}  
Therefore, the expected total regret 
    \begin{align*}
        \rgr{\texttt{UCB},K} \leq \sum_{t=2}^K 2 \sqrt{2\sigma^2\frac{\log(AK/\delta)}{k-1}} + \delta \leq
        \sqrt{2\sigma^2\log(AK/\delta)(K-1)} + K\delta.
    \end{align*} 
Choosing $\delta=1/K$ yields
    \begin{align*}
        \rgr{\texttt{UCB},K} &\leq \sqrt{2\sigma^2\log(AK^2)(K-1)} + \mathcal{O}(1) \\
        &\leq \mathcal{O}(\sigma\sqrt{K\log A})+\mathcal{O}(\sigma\sqrt{K\log K}).
    \end{align*} 
\end{proof}
\subsubsection{Regret bound of Optimistic \pto for tabular Exo-MDP}
\label{sec:pto-opt}
We consider \texttt{PTO-Opt}, an optimistic version of \pto, which replaces the exogenous transition model with its optimistic version. In episode $k$, \texttt{PTO-Opt} performs 
\[
\begin{aligned}
\bar Q^k_h(s_h,a_h)
&:= r(x_h,a_h,\xi_h) + \E_{\xi_{h+1}\mid\xi_h}\bigl[\bar V^k_{h+1}(f(x_h,a_h,\xi_{h+1}),\xi_{h+1});\bar\bP^k\bigr]\\
&=r(x_h,a_h,\xi_h) + \max_{Q_h:\norm{Q_t-\hat{\bP}^k_h(\xi)}_1\leq c_t(\xi)}\sum_{\xi'} Q_h(\xi') \bar V^k_{h+1}(f(x_h,a_h,\xi_{h+1}),\xi_{h+1}),  \\
\bar\pi^k_h(s_h)&\in\arg\max_{a_h}\bar Q^k_h(s_h,a_h),\quad
\bar V^k_h(s_h):=\bar Q^k_h(s_h,\bar\pi^k_h(s_h)).
\end{aligned}
\]
\begin{proposition}[High probability cumulative regret bound of \texttt{PTO-Opt}]
Fix any $\delta \in(0,1)$. With probability at least $1-\delta$, 
$$
\rgr{\texttt{PTO-Opt},K} \leq \cO(H^2 |\Xi|\sqrt{K\log(KH|\Xi|/\delta)}).
$$
\end{proposition}
Compared with Theorem \ref{thm:pto_reg}, \texttt{PTO-Opt} has slightly worse regret bound. This verifies that \pel is sufficient for tabular Exo-MDP with simple implementations.
%\hao{Add proof if time permits}





==> parts/notation.tex <==
\section{Table of Notation}
\label[appendix]{app:not}

\begin{table}[!ht]
\caption{List of common notations.}
\label{tab:notation}
    \centering
    \begin{tabular}{ll}
\toprule
\textbf{Symbol} & \textbf{Definition} \\ \midrule
\multicolumn{2}{c}{{\em Exo-MDP specification}}\\
\hline
$\mathcal{X}$ & Endogenous (system) state space \\
$\Xi$ & Exogenous state space \\
$\mathcal{A}$ & Action space \\
$H$ & Planning horizon \\
$K$ & Number of episodes \\
$x_t \in \mathcal{X}$ & Endogenous state at time $t$ \\
$\xi_t \in \Xi$ & Exogenous input at time $t$ \\
$a_t \in \mathcal{A}$ & Action at time $t$ \\
$f: \mathcal{X}\times \mathcal{A}\times \Xi \to \mathcal{X}$ & Endogenous transition function, $x_{t+1} = f(x_t,a_t,\xi_t)$ \\
$\bP(\xi' \mid \xi)$ & Exogenous transition kernel \\
$r: \mathcal{X}\times \mathcal{A}\times \Xi \to [0,1]$ & Reward function \\
$\pi: \mathcal{X}\times \Xi \to \mathcal{A}$ & Policy mapping state to action \\
$V_h^\pi(x,\xi)$ & Value function of policy $\pi$ at stage $h$ \\
$Q_h^\pi(x,a,\xi)$ & State-action value function of policy $\pi$ at stage $h$ \\
$\mathrm{Regret}(K)$ & Cumulative regret after $K$ episodes \\
\hline
\multicolumn{2}{c}{{\em Pure Exploitation Framework}}\\
\hline
$\texttt{PEL}$ & Pure Exploitation Learning framework \\
$\texttt{FTL}$ & Pure Exploitation algorithm for Exo-bandits ($H=1$) and tabular Exo-MDPs \\
$\texttt{LSVI-PE}$ & Pure Exploitation algorithm for Exo-MDPs with linear function approximation \\
\hline
\multicolumn{2}{c}{{\em LFA}}\\
\hline
$\phi(x)$ & Feature map of state $x$ \\
$d$ & Feature dimension \\
$\theta_h$ & Parameter vector at stage $h$ \\
$\hat P_h$ & Empirical estimate of exogenous transition at stage $h$ \\
$\hat Q_h, \hat V_h$ & Estimated $Q$- and value functions \\
$\iota$ & Logarithmic factor $\log(2KH|\Xi|/\delta)$ in regret bounds \\
\hline
\multicolumn{2}{c}{{\em Storage  Control Example}}\\
\hline
$C$ & Storage capacity \\
$x_h \in [0,C]$ & Storage level at stage $h$ \\
$\xi_h \in \Xi$ & Price at stage $h$ \\
$a_h = (a_h^+, a_h^-)$ & Charge ($a^+$) / discharge ($a^-$) actions \\
$\eta^+, \eta^-$ & Charging/discharging efficiencies \\
$x_h^a$ & Post-decision state after action $a_h$ \\
$\hat \bP(\xi'|\xi)$ & Estimated price transition kernel \\
\hline
\multicolumn{2}{c}{{\em Theoretical Analysis}}\\
\hline
$\delta$ & Confidence parameter in high-probability bounds \\
$N$ & number of anchor points  \\
$\mathcal{O}(\cdot), \tilde{\mathcal{O}}(\cdot)$ & Standard big-$O$ and log-suppressed complexity notation \\
\bottomrule
\end{tabular}
\end{table}

\begin{comment}
\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}
\end{comment}
